Fusing Higher-order Features in Graph Neural Networks for Skeleton-based Action Recognition

Skeleton sequences are lightweight and compact, and thus are ideal candidates for action recognition on edge devices. Recent skeleton-based action recognition methods extract features from 3D joint coordinates as spatial-temporal cues, using these representations in a graph neural network for feature fusion to boost recognition performance. The use of first- and second-order features, i.e., joint and bone representations, has led to high accuracy. Nonetheless, many models are still confused by actions that have similar motion trajectories. To address these issues, we propose fusing higher-order features in the form of angular encoding into modern architectures to robustly capture the relationships between joints and body parts. This simple fusion with popular spatial-temporal graph neural networks achieves new state-of-the-art accuracy in two large benchmarks, including NTU60 and NTU120, while employing fewer parameters and reduced run time. Our source code is publicly available at: https://github.com/ZhenyueQin/Angular-Skeleton-Encoding.

==> letters/letter_1.tex <==
We are delighted to submit our revised manuscript titled \textit{Fusing Higher-Order Features in Graph Neural Networks for Skeleton-Based Action Recognition}. 
First, we sincerely thank all the reviewers and editors for their valuable and constructive comments. 
In this revised manuscript, we have carefully considered the concerns and comments raised by the reviewers and editors. We have addressed all of them in the revised version. We describe our changes here in this letter. 

\noindent 
\textbf{Reviewer \#1}

\noindent 
\textit{1. Please fill the reference e.g., in Introduction (page 1, right column, line 42), Experiment  (page 11, left column, line 1).
}\\
Response: \\
We have filled the references. 

\noindent 
\textit{2. It would be preferred if the authors could explain some concepts in the text. For example, GFlops (Table I and Table V), participants (page 7, right column, line 43). It would help readers from slightly different domains to understand the context.
}\\
Response: \\
We have revised the wording to make the description of the paper more clear. We have explained the meaning of GFlops in both Table I and V as ``GFlop stand for the floating-point operations performed by a model, which is the number of multiply-add operations that a model performs. '' We have also added descriptions for participants ``as the persons conducting actions'' in the revised manuscript. 

\noindent 
\textbf{Reviewer \#2}

\noindent 
\textit{It would have been better if the author had written the angular features in the standard GNN form of message passing so that the reader may comprehend the details more easily.
}\\

The angular encoding is concatenated as a part of the node feature for graph neural networks. The procedures of the GNN are described in Figure 2 and section III.B. We have also further revised the description of the angular encoding in bid to better understanding. For example, we have added further explanation for Eq. (2). 

\noindent 
\textbf{Reviewer \#3}

\noindent 
\textit{1. The novelty of this work is limited. Many works have already investigated the angular features in the skeleton-based action recognition task. What are the main differences between them and the proposed angular features? }\\
Response: \\
We propose a rich collection of various angular encoding forms, including four major categories: (a) local; (b) center-oriented; (c) pair-based; (d) finger-based. Each category consists of further subcategories. Different categories of angular encoding are designed to capture motion features of distinct kinematic body parts. Each category’s angular encoding can independently improve the performance of a skeleton-based action recognizer, as the following table shows. 

We have revised the manuscript by including the following table as Table VI. Furthermore, we have revised the contribution part in the introduction of the paper to make the contributions of angular encoding more clear. 

\begin{tabular}{l|rr|rr}
\toprule 
%\rowcolor{Gray}
Angular Types & \makecell[r]{NTU60\\XSub} & \makecell[r]{NTU60\\XView} & \makecell[r]{NTU120\\XSub} & \makecell[r]{NTU120\\XSet}\\ 
\midrule 
No angular encoding & 87.2 & 93.7 & 81.9 & 83.5 \\ \midrule
With local & 87.9 & 94.1 & 82.8 & 83.5 \\ 
With center-based & 88.4 & 94.3 & 83.0 & 83.7 \\ \midrule
With pair-based & 87.8 & 94.2 & 82.4 & 83.5 \\ 
With finger-based & 88.0 & 94.1 & 82.7 & 83.6\\ \midrule
Concatenating all & 88.7 & 94.5 & 83.2 & 83.7\\ 
\bottomrule
% \hline
% \hline
\end{tabular}

\noindent 
\textit{2. This paper simply makes use of the existing GNN model, and does not make any innovation to promote the development of GNN. What is the novelty of this work about the GNN? Note that the theme of Special Issue is ``Deep Neural Networks for Graphs: Theory, Models, Algorithms and Applications''.}\\
Response: \\
Skeleton-based action recognition is an application of GNN because GNN fuels the recent surge of recognition accuracy. With the exploit of GNN, humans’ topological information can be more thoroughly extracted compared with other neural networks. Our proposed mechanism is widely compatible with existing GNNs of skeleton-based action recognition. This is a contribution to the application of deep neural networks for graphs. 

To make the relevance between the proposed work and graph neural networks more easy-to-follow, we include the following paragraph at the beginning of the paper: 
``Skeleton-based action recognition are more robust to background information and easier to process, attracting increasing attention in the community. Recently, deep graph neural networks fuels the recent surge of accuracy for skeleton-based action recognition. With leveraging graph neural networks, action recognizers more thoroughly extract the topological information within the skeleton sequences. ''

\noindent 
\textit{3. It is claimed that ``our simple yet powerful model employs fewer training parameters and requires less inference time, thus capable of supporting real-time action recognition on edge devices.'' However, this is not the innovation of the proposed method, since the network structure is just a simplified version of the existing MSG3D. }\\
Response: \\
We aim to express the power of the proposed angular encoding for accuracy uptick. We change the wording as: ``If a simple model (employing fewer training parameters and requiring less inference time) has equipped with the proposed angular encoding, it becomes powerful. Thus, the proposed angular encoding supports real-time action recognition on edge devices''. 

\noindent 
\textit{4. Although this paper reviews the graph neural network-based methods in Related Work, many relevant references, especially the state-of-the-art methods in recent years, are missing and should be included.}\\
Response: \\
We have included various methods that were proposed more recently in the related work section. The paragraph is as follows: 
``In more recent time, Qin \etal proposed some self-attention models that dynamically optimize the graph structure (2022). Xu \etal designed a pure CNN architecture that more effectively capture the topological information (2021). Memmesheimer \etal study the one-shot problem of skeleton-based action recognition (2022). They apply the metric learning setting and maps the problem to a nearest-neighbor search in a set of activity reference samples. Wang \etal studied the adversarial attack problem in skeleton-based action recognition (2021). They investigated a perceptual loss that ensures the imperceptibility of the attack. Diao \etal investigated the black-box attack on skeleton-based action recognition (2021). They proposed an attack mechanism called BASKR and showed that the adversarial attack is a threat since on-manifold adversarial adversarial samples are common for skeletal motions. ''. 

\noindent 
\textit{5. Although the focus is on designing angular encoding, I see no discussion of the existing angular features for the skeleton-based action recognition task in the Introduction and Related Work. The author should discuss and give the theoretical comparison with respect to the existing angular features. }\\
Response: \\
We discover two papers published in the year of 2022 that have angle features. We list the comparison in the end of the related work part as follows: 
``Some work exhibit angle features similar to the local feature presented in this paper (see the main paper for citations). On the other hand, we propose a rich collection of various angular encoding forms. Each category consists of further subcategories. Different categories of angular encoding are designed to capture motion features of distinct kinematic body parts''. We also give theoretical comparison from the hypergraph perspective. 

\noindent 
\textit{6. The description in section III-B is not clear. Though this paper uses the existing model (MSG3D), the details of the network architecture should be given, since it is difficult to follow and understand.}\\
Response: \\
We have revised the wording in section III-B to make the explanation more clear. We include Figure 3 that demonstrates the details of the network architecture. 

\noindent 
\textit{7. The motivation and the effectiveness of the proposed method is mainly demonstrated by experimental performance. It is more convincing if the authors could give more theoretical analysis.}\\
Response: \\
We have given theoretical analysis from the hypergraph perspective in the discussion section, such as the following paragraph: 
``As we have described in the introduction, current GCNs are designed to extract features between two adjacent nodes. On the other hand, the angular features, is a higher-order feature beyond two adjacent vertices. We can theoretically view every angle as a hyperedge $e(v_1, v_2, v_3)$, where $v_1$, $v_2$ and $v_3$ are the constitutional joints of an angle. The angular encoding is their associated features. The angular encoding extends the capability of existing GNNs to be able to capture features of hyperedges''.  

\noindent 
\textit{8. The rationality and the effectiveness of the Eq. (2) should be further explained.}\\
Response: \\
We have presented more rationality description following the Eq. (2), such as: ``The angular encoding is a third-order feature. Taking the velocity of these third-order features further increase the order. Hence, these velocity angular features enable an skeleton-based action recognizer to capture fourth-order information of skeleton motion sequences''. 

As for the effectiveness, qe give the experimental results of using the angular velocity alone in table II. Furthermore, when combing the joint velocity feature with the angular velocity feature, the accuracy improves from 79.31\% to 83.81\%. This huge increase (more than 4\%) demonstrates the effectiveness of the angular velocity shown in Eq. (2). 

\noindent 
\textit{9. More datasets should be used to validate the performance of the proposed method. }\\
Response: \\
In ICCV 2021, the winning team of the skeleton-based action recognition stream leveraged our angular encoding, achieving the 1st-place accuracy among 70+ teams. The utilized dataset was a newly collected skeleton dataset with drones. The winning team specifically evaluated the boost of accuracy from using our proposed angular encoding on the newly recorded dataset, showing the effectiveness of angular encoding. See their  \href{https://sutdapac-my.sharepoint.com/:v:/g/personal/jun_liu_sutd_edu_sg/EYL7JHl-f2FPvo95wmyoX88Bp_pn71wjgv6J4uiIZGACeA?e=UfLYPs}{presentation (clickable)} (8:30). 
We include this part as a footnote in the experiment part. 

\noindent 
\textit{10. To further examine the performance, the authors should add more state-of-the-art compared methods in recent years, such as the methods proposed in 2021 and 2022.}\\
Response: We have compared with more approaches that were proposed in 2021 and 2022. See Table I for details. 

\noindent 
\textit{11. There are many mistakes, such as “STGCN [31], ShiftGCN [] and DecoupleGCN []” in the right of Page 1.
}\\
Response: We have filled the missing citations. We also have revised other places. 

\noindent 
\textit{12. The full spelling of abbreviation should be given at the first time, e.g., STGCN.
}\\
Response: We have given the full names of the abbreviations shown for the first time. 

\noindent 
\textit{13. Some references on GNNs are missing. 
}\\
Response: We have substantially benefited from reading the provided references. We have cited them since they help enrich the scope of this paper. 



==> recycle/recycle.tex <==
\begin{table*}[t]
\rowcolors{1}{Lavender!80!gray}{white}
\centering
\caption{Confusion matrix. } 
% \vspace{-2mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\hline\hline 
 \multicolumn{2}{l}{Actions} & 
 \multicolumn{2}{l}{Staple\\books} & 
 \multicolumn{2}{l}{Make OK/\\victory sign} & 
 \multicolumn{2}{l}{Thumb\\up/down} & 
 \multicolumn{2}{l}{Open\\a box} & 
 \multicolumn{2}{l}{Blow\\nose} & 
 \multicolumn{2}{l}{Shaking\\fist} & 
 \multicolumn{2}{l}{Take off\\headphone} & 
 \multicolumn{2}{l}{Cross heads\\in front} & 
 \multicolumn{2}{l}{Sitting\\down} & 
 \multicolumn{2}{l}{Hit person\\with sth.} &
 \multicolumn{2}{l}{Typing\\on keyboard} & 
 \multicolumn{2}{l}{Sniff\\(Smell)} \\ \hline 
 \makecell[l]{Jnt\\Acc (\%)} & 0.31 & \makecell[c]{0.41/\\0.35} & \makecell[c]{0.64/\\0.83} & 0.68 & 0.59 & 0.76 & 0.84 & 0.92 & 0.93 & 0.6 & 0.68 & 0.78 \\ \hline 
 \makecell[l]{Ang\\Acc (\%)} & 0.42 & \makecell[c]{0.49/\\0.48} & \makecell[c]{0.73/\\0.86} & 0.76 & 0.66 & 0.82 & 0.87 & 0.94 & 0.95 & 0.62 & 0.69 & 0.79 \\ \hline
 \makecell[l]{Jnt most\\confused with} & 
 \makecell[c]{Cutting\\paper} & 
 \makecell[c]{Make victory/\\OK sign} & 
 \makecell[c]{Thumb\\down/up} & 
 \makecell[c]{Open\\a bottle} & 
 \makecell[c]{Hush\\(quiet)} & 
 \makecell[c]{Hand-\\waving} & 
 \makecell[c]{Take off\\glasses} & 
 \makecell[c]{Take a\\selife} & 
 \makecell[c]{Falling} & 
 \makecell[c]{Wield knife\\toward other person} &
 \makecell[c]{Writing} & 
 \makecell[c]{Blow\\nose} \\ \hline 
 \makecell[l]{Ang most\\confused with} & 
 \makecell[c]{Cutting\\paper} & 
 \makecell[c]{Make victory/\\OK sign} & 
 \makecell[c]{Thumb\\down/up} & 
 \makecell[c]{Open\\a bottle} & 
 \makecell[c]{Yawn} & 
 \makecell[c]{Hand-\\waving} & 
 \makecell[c]{Flick hair} & 
 \makecell[c]{Put the\\palms together} & 
 \makecell[c]{Squat\\down} & 
 \makecell[c]{Wield knife\\toward other person} &
 \makecell[c]{Writing} & 
 \makecell[c]{Blow\\nose} \\ \hline\hline
\end{tabular}
}
\label{Tab:Scale}
\end{table*}


\begin{table*}[t]
\centering
\caption{Compare with SOTA. } 
% \vspace{-2mm}
\begin{tabular}{lcccccccc}
\hline
\hline
% row 1
\rowcolor{Gray}
&
&
\multicolumn{2}{c}{NTU} 
& \multicolumn{2}{c}{NTU120}
& \multicolumn{2}{c}{Kinetics}
& stream
\\
% row 2
\rowcolor{Gray}
&
\multirow{-2}{*}{Venue} &
X-Sub
& X-View
& X-Sub
& X-Set
& Top-1 & Top-5 
& Num
\\
\hline 
ST-GCN~\cite{yan2018spatial} & AAAI & 81.5 & 88.3 & - & - & 30.7 & 52.8 & Jnt
\\ 
% DPRL~\cite{tang2018deep} & 83.5 & 89.8 & - & - & - & - \\ 
HCN~\cite{li2018co} & IJCAI & 86.5 & 91.1 & - & - & - & - & Jnt
\\ 
MAN~\cite{xie2018memory} & IJCAI & 82.7 & 93.2 & - & - & - & - & Jnt
\\ 
AS-GCN~\cite{li2019actional} & CVPR & 86.8 & 94.2 & - & - & 34.8 & 56.5 & Jnt
\\
AGC-LSTM~\cite{si2019attention} & CVPR & 89.2 & 95.0 & - & - & - & - & Jnt; Part
\\
2s-AGCN~\cite{shi2019two} & CVPR & 88.5 & 95.1 & - & - & 36.1 & 58.7 & Jnt; Bon \\
DGNN~\cite{shi2019skeleton} & CVPR & 89.9 & 96.1 & - & - & 36.9 & 59.6 & Jnt; Bon \\
Bayes-GCN~\cite{zhao2019bayesian} & ICCV & 81.8 & 92.4 & - & - & - & - & Jnt \\
SGN~\cite{zhang2020semantics} & CVPR & 89.0 & 94.5 & 79.2 & 81.5 & - & - & Jnt; Vel \\
Shift-GCN~\cite{cheng2020skeleton} & CVPR & 90.7 & 96.5 & 85.9 & 87.6 & - & - &  \\
DeCoup-GCN~\cite{chengdecoupling} & ECCV & 90.8 & 96.6 & 86.5 & 88.1 & - & - \\
MS-G3D~\cite{liu2020disentangling} & CVPR & 91.5 & 96.2 & 86.9 & 88.4 & 38.0 & 60.9 \\
\hline 
\ourmodel-JA (Cct: Jnt + Ang) & - & & & & & \\
\ourmodel-BA (Cct: Bon + Ang) & - & & & & & \\
\ourmodel-JBA: (Cct: Jnt + Bon + Ang) & - & & & & & \\
\ourmodel-VJBA: (Cct: Jnt + Bon + Ang) & - & & & & & \\
\hline 
Ens-2: \ourmodel-JBA + VJBA & - & 91.0 & 96.1 &  87.6 & 88.8 & & \\
Ens-4: \ourmodel-JA + BA + JBA + VJBA & - & 91.7 & 96.4 &  88.2 & 89.2 & &  \\
\hline
\hline
\end{tabular}
\label{Tab:Scale}
\end{table*}

\begin{table*}[t]
\centering
\caption{Compare with SOTA. } 
% \vspace{-2mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccrr}
\hline
\hline
% row 1
\rowcolor{Gray}
&
&
Ens &
\multicolumn{2}{c}{NTU} 
& \multicolumn{2}{c}{NTU120}
& \multicolumn{2}{c}{Kinetics}
& Param
& 
\\
% row 2
\rowcolor{Gray}
&
\multirow{-2}{*}{Venue} &
Num &
X-Sub
& X-View
& X-Sub
& X-Set
& Top-1 & Top-5 
& Num
& \multirow{-2}{*}{GFlops}
\\
\hline 
% DPRL~\cite{tang2018deep} & 83.5 & 89.8 & - & - & - & - \\ 
HCN~\cite{li2018co} & IJCAI & 1 & 86.5 & 91.1 & - & - & - & - & - & -
\\ 
MAN~\cite{xie2018memory} & IJCAI & 1 & 82.7 & 93.2 & - & - & - & - & - & -
\\ 
ST-GCN~\cite{yan2018spatial} & AAAI & 1 & 81.5 & 88.3 & - & - & 30.7 & 52.8 & 2.91M & 16.4
\\ 
AS-GCN~\cite{li2019actional} & CVPR & 1 & 86.8 & 94.2 & - & - & 34.8 & 56.5 & 7.17M & 35.5
\\
AGC-LSTM~\cite{si2019attention} & CVPR & 2 & 89.2 & 95.0 & - & - & - & - & - & -
\\
2s-AGCN~\cite{shi2019two} & CVPR & 4 & 88.5 & 95.1 & - & - & 36.1 & 58.7 & 6.72M & 37.2
\\
DGNN~\cite{shi2019skeleton} & CVPR & 4 & 89.9 & 96.1 & - & - & 36.9 & 59.6 & 8.06M & 71.1
\\
Bayes-GCN~\cite{zhao2019bayesian} & ICCV & 1 & 81.8 & 92.4 & - & - & - & - & - & -
\\
SGN~\cite{zhang2020semantics} & CVPR & 1 & 89.0 & 94.5 & 79.2 & 81.5 & - & - & 0.69M & 15.4
\\
Shift-GCN~\cite{cheng2020skeleton} & CVPR & 4 & 90.7 & 96.5 & 85.9 & 87.6 & - & - & 2.77M & 19.2
\\
DeCoup-GCN~\cite{chengdecoupling} & ECCV & 4 & 90.8 & 96.6 & 86.5 & 88.1 & - & - & 13.72M & 102.3
\\
MS-G3D~\cite{liu2020disentangling} & CVPR & 2 & 91.5 & 96.2 & 86.9 & 88.4 & 38.0 & 60.9 & 6.44M & 98.0
\\
\hline 
Cct: \ourmodel-JA (Jnt + Ang) & Ours & 1 & 88.7 & 94.5 & 83.6 & 83.7 & & & 1.46M & 19.6 \\
Cct: \ourmodel-BA (Bon + Ang) & Ours & 1 & 89.2 & 94.8 & 84.6 & 85.5 & & & 1.46M & 19.6 \\
Cct: \ourmodel-JBA: (Jnt + Bon + Ang) & Ours & 1 & 90.0 & 94.8 & 85.9 & 86.8 & & & 1.50M & 20.6 \\
Cct: \ourmodel-VJBA: (Jnt + Bon + Ang) & Ours & 1 & 87.1 & 94.0 & 83.0 & 84.6 & & & 1.50M & 20.6 \\
% \hline 
Fuse: \ourmodel-JBA + VJBA & Ours & 2 & 91.0 & 96.1 &  87.6 & 88.8 & & & 3.00M & 41.2 \\
Fuse: \ourmodel-BA + JBA + VJBA & Ours & 3 & 91.6 & 96.3 &  88.4 & 89.1 & & & 4.38M & 60.8 \\
% Fuse: \ourmodel-JA + BA + JBA + VJBA & Ours & 4 & 91.7 & 96.4 &  88.2 & 89.2 & & & 5.84M \\
\hline
\hline
\end{tabular}
}
\label{Tab:Scale}
\end{table*}

\begin{table*}[t]
\centering
\caption{Confusion matrix. } 
% \vspace{-2mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\hline\hline 
 \rowcolor{Gray}
 & Staple 
 & Make OK/ 
 & Thumb 
 & Open 
 & Blow 
 & Shaking 
 & Take off 
 & Cross heads 
 & Sitting 
 & Hit person 
 & Typing 
 & Sniff \\
 \rowcolor{Gray}
 \multirow{-2}{*}{Actions} 
 & books 
 & victory sign 
 & up/down 
 & a box 
 & nose 
 & fist 
 & headphone 
 & in front 
 & down 
 & with sth. 
 & on keyboard 
 & (smell) \\
 \hline 
 \rowcolor{Gray!30}
 Jnt 
 & 
 & 0.41
 & 0.65 
 & & & & & & & & & \\
 \rowcolor{Gray!30}
 Acc (\%) 
 & \multirow{-2}{*}{0.31}
 & 0.35
 & 0.83 
 & \multirow{-2}{*}{0.68}
 & \multirow{-2}{*}{0.59}
 & \multirow{-2}{*}{0.76}
 & \multirow{-2}{*}{0.84}
 & \multirow{-2}{*}{0.92}
 & \multirow{-2}{*}{0.93}
 & \multirow{-2}{*}{0.6}
 & \multirow{-2}{*}{0.68}
 & \multirow{-2}{*}{0.78} \\

 Jnt most 
 & Cutting
 & Make victory/
 & Make victory sign/
 & Open
 & Hush
 & Hand-
 & Take off
 & Take a
 & 
 & Wield knife
 & 
 & Hush\\

 confused with
 & paper
 & ok sign
 & thumb up
 & a bottle
 & (quiet)
 & waving
 & glasses
 & selife
 & \multirow{-2}{*}{Falling}
 & toward other person
 & \multirow{-2}{*}{Writing}
 & (quite) \\ \hline 
 
 \rowcolor{Gray!30}
 Ang 
 & 
 & 0.49
 & 0.73
 & & & & & & & & & \\
 \rowcolor{Gray!30}
 Acc (\%) 
 & \multirow{-2}{*}{0.42}
 & 0.48
 & 0.86
 & \multirow{-2}{*}{0.76}
 & \multirow{-2}{*}{0.66}
 & \multirow{-2}{*}{0.82}
 & \multirow{-2}{*}{0.87}
 & \multirow{-2}{*}{0.94}
 & \multirow{-2}{*}{0.95}
 & \multirow{-2}{*}{0.62}
 & \multirow{-2}{*}{0.69}
 & \multirow{-2}{*}{0.79} \\

 Ang most 
 & Cutting
 & Make victory/
 & Thumb
 & Open
 & 
 & Hand-
 & Flick
 & Put the
 & Squat
 & Wield knife
 & 
 & Blow
 \\
 confused with
 & paper
 & ok sign
 & down/up
 & a bottle
 & \multirow{-2}{*}{Yawn}
 & waving
 & hair
 & palms together
 & down
 & toward other person
 & \multirow{-2}{*}{Writing}
 & nose \\ \hline \hline 
\end{tabular}
}
\label{Tab:Scale}
\end{table*}

==> secs/different_angular_copy.tex <==
\section{Different Angles}

\begin{table}[t]
\centering
% \vspace{-2mm}
% \resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|rr|rr}
\toprule 
%\rowcolor{Gray}
Features & Static & Acc$\uparrow$ (\%) & Velocity & Acc$\uparrow$ (\%) \\ 
\midrule 
\rowcolor{Gray!30}
Jnt & 81.90 & -- & 79.31 & -- \\ 
Cct: Jnt + Local & 82.25 & 0.35 & 80.04 & 0.73 \\
Cct: Jnt + Center & 82.91 & 1.01 & 81.33 & 2.02 \\
Cct: Jnt + Part & 82.12 & 0.22 & 80.78 & 1.47 \\
Cct: Jnt + Finger & 82.63 & 0.73 & 80.76 & 1.45 \\
\bottomrule 
\end{tabular}
% }
\caption{Evaluation results on the concatenation of angular features. Cct indicates the concatenation. The red bold number highlights the highest prediction accuracy. Acc$\uparrow$ is the improvment in accuracy. } 
% \vspace{-4.95mm}
\label{table:dif_ang_imp}
\end{table}

\begin{table*}[t]
% \vspace{-2mm}
% Subtable 1
\begin{subtable}[t]{0.99\textwidth}
\centering
\caption{Actions whose accuracy values are boosted by the local angular feature. }
% \resizebox{\textwidth}{!}{
\begin{tabular}{c|l|rc|rrc}
\toprule 
%\rowcolor{Gray}
& & \multicolumn{2}{c|}{\textbf{Joint}} & \multicolumn{3}{c}{\textbf{Concatenation: Joint + Angular}} \\
\cline{3-4}\cline{5-7}
%\rowcolor{Gray}
& \multirow{-2}{*}{\textbf{Action}} & Acc (\%) & Similar Action & Acc (\%) & Acc$\uparrow$ (\%) & Similar Action \\ 
\midrule 
\multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{Static}}} 
& take off a shoe & 72.63 & wear a shoe & 80.67 & 12.04 & wear a shoe \\
& use a fan &	83.27 & hand waving & 90.55	& 7.27 & shake fist \\
& staple book & 27.32 & cutting paper & 36.08 & 8.76 & cutting paper \\
& fold paper & 60.35 & ball up paper & 66.78 & 6.43 & open a box \\
& counting money & 47.72 & play magic cube & 54.04 & 6.32 & play magic cube \\
% & wipe face & 82.25 & brushing hair & 88.41 & 6.16 & apply cream on face \\
% & kicking other person & 88.04 & step on foot & 91.3 & 3.26 & side kick \\
% & wield knife towards other person & 64.24 & hit other person with something & 68.92 & 4.69 & hit other person with something \\
% & pointing to something with finger & 72.46 & taking a selfie & 76.45 & 3.99 & taking a selfie \\
% & touch head & 78.26 & brushing teeth & 81.88 & 3.62 & blow nose \\
\midrule
\multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{Velocity}}} 
% & make victory sign & 36.87 & make ok sign & 49.22 & 12.35 & make ok sign \\
& cutting paper (using scissors) & 35.78 & staple book & 45.90 & 10.12 & staple book \\
& writing & 54.04 & typing on a keyboard & 61.76 & 7.72 & typing on a keyboard \\
% & drop & 78.18 & sniff (smell) & 84.73 & 6.55 & sniff (smell) \\
& fold paper & 57.22 & ball up paper & 63.48 & 6.26 & counting money \\
& take a photo of other person & 84.03 & shoot at other person with a gun & 89.93 & 5.9 & shoot at other person with a gun \\
& typing on a keyboard & 61.82 & writing & 67.27 & 5.45 & writing \\
\bottomrule 
\end{tabular}
% }
\end{subtable}

% Subtable 2
\begin{subtable}[t]{0.99\textwidth}
\centering
\caption{Actions whose accuracy values are boosted by the center-oriented angular feature. }
% \resizebox{\textwidth}{!}{
\begin{tabular}{c|l|rc|rrc}
\toprule 
%\rowcolor{Gray}
& & \multicolumn{2}{c|}{\textbf{Joint}} & \multicolumn{3}{c}{\textbf{Concatenation: Joint + Angular}} \\
\cline{3-4}\cline{5-7}
%\rowcolor{Gray}
& \multirow{-2}{*}{\textbf{Action}} & Acc (\%) & Similar Action & Acc (\%) & Acc$\uparrow$ (\%) & Similar Action \\ 
\midrule 
\multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{Static}}} 
& make victory sign & 17.22 & make ok sign & 40.35 & 23.13 & make ok sign \\ 
& playing with phone/tablet & 54.55 & play magic cube & 68.36 & 13.82 & play magic cube \\
& take something out of a bag & 78.3 & put something into a bag & 85.94 & 7.64 & put something into a bag \\
& fold paper & 59.83 & open a box & 66.09 & 6.26 & counting money \\
& counting money & 45.26 & play magic cube & 51.4 & 6.14 & play magic cube \\
% & open bottle & 65.97 & play magic cube & 71.9 & 5.93 & play magic cube \\
% & brushing hair & 86.45 & touch head & 91.94 & 5.49 & wipe face \\
% & brushing teeth & 79.49 & touch head & 84.62 & 5.13 & drink water \\
% & typing on a keyboard & 61.45 & writing & 66.55 & 5.09 & writing \\
% & exchange things with other person & 85.74 & giving something to other person & 89.91 & 4.17 & giving something to other person \\ \bottomrule 
\midrule 
\multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{Velocity}}} 
& cutting paper (using scissors) & 35.78 & staple book & 58.12 & 22.34 & staple book \\
& check time (from watch) & 80.43 & cross hands in front (say stop) & 89.49 & 9.06  & tear up paper \\
& typing on a keyboard & 61.82 & writing & 70.18 & 8.36 & writing \\
& open bottle & 65.1 & open a box & 72.43 & 7.33 & open a box \\
& counting money & 46.84 & play magic cube & 53.86 & 7.02 & play magic cube \\
\bottomrule
\end{tabular}
% }
\end{subtable}

% Subtable 3 
\begin{subtable}[t]{0.99\textwidth}
\centering
\caption{Actions whose accuracy values are boosted by the part-based angular feature. }
% \resizebox{\textwidth}{!}{
\begin{tabular}{c|l|rc|rrc}
\toprule 
%\rowcolor{Gray}
& & \multicolumn{2}{c|}{\textbf{Joint}} & \multicolumn{3}{c}{\textbf{Concatenation: Joint + Angular}} \\
\cline{3-4}\cline{5-7}
%\rowcolor{Gray}
& \multirow{-2}{*}{\textbf{Action}} & Acc (\%) & Similar Action & Acc (\%) & Acc$\uparrow$ (\%) & Similar Action \\ 
\midrule
\multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{Static}}} 
& make victory sign & 17.22 & make ok sign & 37.39 & 20.17 & make ok sign \\
% nausea or vomiting condition & 76.36 & touch chest (stomachache/heart pain) & 86.18 & 9.82 & touch chest (stomachache/heart pain) \\
& counting money & 45.26 & play magic cube & 54.56 & 9.3 & play magic cube \\
& brushing teeth & 79.49 & touch head (headache) & 88.28 & 8.79 & drink water \\
& shake fist & 71.7 & hand waving & 78.47 & 6.77 & hand waving \\ 
& hopping (one foot jumping) & 92 & staggering & 96.73 & 4.73 & staggering \\
% & hit other person with something & 58.61 & wield knife towards other person & 63.13 & 4.52 & wield knife towards other person \\
% & grab other person's stuff & 85.39 & wield knife towards other person & 89.91 & 4.52 & hit other person with something \\
% & take something out of a bag & 78.3 & put something into a bag & 81.94 & 3.65 & put something into a bag \\
% & pointing to something with finger & 73.55 & taking a selfie & 77.17	& 3.62 & taking a selfie \\
% & take off jacket & 92.39 & take off bag & 96.01 & 3.62 & wear jacket \\
\midrule
\multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{Velocity}}}
& cutting paper (using scissors) & 35.78 & staple book & 59.34 & 23.56 & staple book  \\
& brushing teeth & 77.29 & drink water & 88.28 & 10.99 & drink water \\
& check time (from watch) & 80.43 & cross hands in front (say stop) & 90.94 & 10.51 & taking a selfie \\
& typing on a keyboard & 61.82 & writing & 72.00 & 10.18 & writing \\
& open a box & 59.23 & open bottle & 68.82 & 9.58 & open bottle \\
% & play magic cube & 58.57 & playing with phone/tablet & 64.86 & 6.29 & counting money \\
\bottomrule 
\end{tabular}
% }
\end{subtable}

% Subtable 4
\begin{subtable}[t]{0.99\textwidth}
\centering
\caption{Actions whose accuracy values are boosted by the finger-based angular feature. }
% \resizebox{\textwidth}{!}{
\begin{tabular}{c|l|rc|rrc}
\toprule 
%\rowcolor{Gray}
& & \multicolumn{2}{c|}{\textbf{Joint}} & \multicolumn{3}{c}{\textbf{Concatenation: Joint + Angular}} \\
\cline{3-4}\cline{5-7}
%\rowcolor{Gray}
& \multirow{-2}{*}{\textbf{Action}} & Acc (\%) & Similar Action & Acc (\%) & Acc$\uparrow$ (\%) & Similar Action \\ 
\midrule
\multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{Static}}} 
& make victory sign & 17.22 & make ok sign & 47.13 & 29.91 & thumb up \\
& shake fist & 71.70 & hand waving & 80.56 & 8.85 & hand waving \\ 
& counting money & 45.26 & play magic cube & 52.63 & 7.37 & play magic cube \\
& snapping fingers & 58.54 & thumb up & 65.68 & 7.14 & shake fist \\
% & pointing to something with finger & 73.55 & taking a selfie & 80.43 & 6.88 & taking a selfie \\
& exchange things with other person & 85.74 & giving something to other person & 89.91 & 6.87 & giving something to other person \\
% open bottle & 65.97 & play magic cube & 72.6 & 6.63 & play magic cube \\
% eat meal & 67.27 & drink water & 73.09 & 5.82 & brushing teeth \\
% brushing teeth & 79.49 & touch head (headache) & 84.98 & 5.49 & 	touch head (headache) \\ 
% playing with phone/tablet & 54.55 & play magic cube & 60 & 5.45 & 	apply cream on hand back \\
% cutting paper (using scissors) & 62.13 & staple book & 66.84 & 4.71 & staple book \\
% hit other person with something & 58.61 & wield knife towards other person & 62.96 & 4.35 & wield knife towards other person \\
\midrule
\bottomrule 
\end{tabular}
% }
\end{subtable}

\caption{
A comparison of the effect for improving action recognition by concatenating certain angular feature to the joint representation. Each subtable is sorted by the increase of accuracy.  
The `Action' column shows the ground truth labels, and the `Similar Action' column shows the predictions from the model (with/without angular features).
The accuracy improvements highlighted in red are the substantially increased ones (Acc$\uparrow$ $\geq$ 10\%) due to using our angular features.
} 
\label{table:confusion}
\end{table*}

% We have demonstrated in section x the effectiveness of the angular encoding on improving the accuracy of recognizing skeleton based actions. Furthermore, we have shown in section x that angular encoding consistently improves accuracy on three different backbone architectures, indicating generalisability. 

In this section, we conduct ablation studies on different types of the proposed angular encoding for improving the accuracy of recognizing skeleton-based actions. The baseline accuracy is obtained merely using the joint feature. Then, we concatenate different types of angular encoding with the joint feature to evaluate the effectiveness of each encoding type. 



We study the effects of different types of angular features on improving the accuracy of recognizing actions. As depicted in 

==> secs/intro_old.tex <==
\section{Introduction}
Action recognition (AR) is a long-standing problem in pattern recognition. It has many useful real-world applications such as smart video surveillance, human computer interaction, sports analysis and health care. Compared to the use of conventional RGB-based models, skeleton-based AR methods are more robust to background noise and they are cheaper and easier to process, which attracts the vision community. Moreover, mobile devices for human pose estimation are readily available with decreasing prices, which increases their suitability for the use in edge devices for real-time AR.

\begin{figure}[ht]
\centering
\begin{subfigure}{.23\textwidth}
  \centering
  % include first image
  \includegraphics[width=.99\linewidth]{imgs/illustrations/cv2_processed_img_glasses.png}  
  \caption*{Taking off glasses. }
  \label{fig:off_headphone}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{imgs/illustrations/cv2_processed_img_headphone.png}  
  \caption*{Taking off headphones. }
  \label{fig:off_glass}
\end{subfigure}
\caption{Sample skeletons with similar motion trajectories: (left) taking off glasses vs (right) taking off headphones. Blue solid lines represent the bones and red dashed lines are the angles shaped by the fore- and upper arm when performing the actions. }
\label{fig:skeleton_off_glass_headphone}
\end{figure}

Skeleton sequences have 3 main characteristics that make them still quite popular in AR: (i) strong correlations between each body joint and its adjacent body joints so that the each skeleton sequence contains very rich body structural information; (ii) temporal continuity exists not only in the same body joint but also in the body structure; (iii) the co-occurrence relationship between spatial and temporal domains.

In recent skeleton-based AR work, skeletons are treated as graphs, with each vertex representing each body joint and each edge is treated as bone. Initially, only the first-order features were employed, representing the coordinates of the joints. Subsequently, \cite{shi2019two} introduced a second-order feature where each joint is represented as the relative joint differences between each pair of joints w.r.t. its nearest neighbors. The experimental results show that their second-order feature representation improves the AR accuracy.

In~\cite{Si_2019_CVPR}, an attention enhanced graph convolutional LSTM network (AGC-LSTM) is proposed for AR from skeleton data. The proposed model can not only capture discriminative features in spatial configuration and temporal dynamics but also explore the co-occurrence relationship between spatial and temporal domains. Moreover, to select discriminative spatial information, the key body joints in each AGC-LSTM layer is enhanced through the attention mechanism. In~\cite{Li_2019_CVPR}, to capture richer dependencies, they introduce an encoder-decoder structure, called A-links inference model, to capture action-specific latent dependencies (or say, capture the latent dependencies between any joints), i.e. actional links, directly from actions. Then they extend the skeleton graphs to represent higher order relationships as the structural links (S-links). They further propose the actional-structural graph convolution network (AS-GCN) that stacks actional-structural graph convolution and temporal convolution as a basic building block, to learn both spatial and temporal features for AR.

Motivated by most recent skeleton-based AR, we propose to use the third-order feature representation in the form of angular features. Our results suggest that the proposed angular features allow the model to more precisely recognize actions. Angle information between informative human body joints capture not only the spatial cues per video frame but also the temporal dependence and relationships within the video sequence. We think that by fusing this angular information into the existing modern AR architectures, such as ST-GCN, SCK + DCK, challenging actions can be classified much easier, especially when the actions have very close motion trajectories (see ~\autoref{fig:skeleton_off_glass_headphone}). 
% However, the angles between the fore- and upper arms differ somewhat more (\dw{can we say these angles are 'very' different to compare with the difference between coordinates? - would be better to say something like angles can give more discriminative information in certain scenarios.)}. 
% However, the angles between the fore- and upper arms are more discriminative, as \autoref{fig:skeleton_off_glass_headphone} exhibits. 

{\bf --- needs update for the paragraph ---}

% It would be possible to input all third-order angle features to a learning system; however, the number of features would be immense, as we discuss subsequently. Instead, we propose a limited set of angular features that are directly relevant to recognizing actions. Our experimental results demonstrate their consistent efficacy in recognizing actions, either by concatenating the new angular features with previously-used features, or by training a new model using the angular representations as the sole input, and then ensembling the resulting classifier with systems using those previous features.

% \rim{I think it's probably best to put this first (asee above). 
% One may wonder whether it is possible to design a neural network to implicitly learn the angular features. We show later in the paper that such design is} 
% \dw{beyond the capability of the current networks (over-claim if you don't have any proof. i guess they can learn angular features, but the sample complexity is just too high.)}. 

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{imgs/skeletons/skeletons.pdf}
    \caption{Examples of Angular Features}
    \label{fig:skeletons}
\end{figure*}

It is worth considering whether it is possible to design a neural network to implicitly learn the angular features. We show later in the paper that such \SA{a} design is challenging for current neural network models. In brief, there are two reason\SA{s}. \st{Firstly,} \SA{i)} Graph neural networks are currently the best-performing models in classifying skeleton-based actions. To model the relationships among all the joints, a graph network requires many iterations of message passing and aggregation. However, recent work implies the performance of GNNs \SA{GNNs??} can be compromised by using more layers\st{,}\SA{;} the problem being known as over-smoothing~\cite{min2020scattering}. \st{Secondly,} \SA{ii)} Modern graph networks learn the relationships among nodes via an adjacency matrix, which only captures pairwise relevance, whereas angles are third-order relationships\st{,} involving three joints. 


{\bf --- needs update for the above paragraph ---} 


We summarize our contributions as follows: 
\begin{enumerate}
    \item We propose a third-order representation using the angular features. Our ablation studies demonstrate its robustness and efficiency in skeleton-based AR.
    \item The angular features we propose can be easily fused into existing modern AR architectures to further boost the recognition performance. Our experiments show that the angular features are complementary information in terms of existing features i.e., relative joint position differences.
    \item We are the first to incorporate the angular features into modern spatio-temporal GCNs that achieves the state-of-the-art results on several benchmarks including NTU120 and Kinetics dataset. Meanwhile, our simple yet powerful model enjoys fewer training parameters thus supporting real-time AR.
\end{enumerate}


==> secs/methods_old.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=.99\linewidth]{imgs/nets/Architecture.pdf}
    \caption{net architecture}
    \label{fig:net_architecture}
\end{figure*} is 
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{imgs/skeletons/skeletons.pdf}
    \caption{Caption}
    \label{fig:my_label}
\end{figure*}

% \begin{figure*}[ht]
% \centering
% \begin{subfigure}{.10\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=.99\linewidth]{imgs/skeletons/skeleton_local.png}  
%   \captionsetup{justification=centering}
%   \caption{Local Bone}
%   \label{subfig:local_bone}
% \end{subfigure}
% \begin{subfigure}{.10\textwidth}
%   \centering
%   % include second image
%   \includegraphics[width=.99\linewidth]{imgs/skeletons/skeleton_center_1.png}  
%   \captionsetup{justification=centering}
%   \caption{Center\\Joint}
%   \label{subfig:center_joint}
% \end{subfigure}
% \begin{subfigure}{.10\textwidth}
%   \centering
%   % include second image
%   \includegraphics[width=.99\linewidth]{imgs/skeletons/skeleton_center_2.png}  
%   \captionsetup{justification=centering}
%   \caption{Center\\Axis}
%   \label{subfig:center_axis}
% \end{subfigure}
% \begin{subfigure}{.10\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=.99\linewidth]{imgs/skeletons/skeleton_two_hands.png}  
%   \captionsetup{justification=centering}
%   \caption{Part\\Hand}
%   \label{subfig:two_hands}
% \end{subfigure}
% \begin{subfigure}{.10\textwidth}
%   \centering
%   % include second image
%   \includegraphics[width=.99\linewidth]{imgs/skeletons/skeleton_two_elbows.png}  
%   \captionsetup{justification=centering}
%   \caption{Part\\Elbow}
%   \label{subfig:two_elbows}
% \end{subfigure}
% \begin{subfigure}{.10\textwidth}
%   \centering
%   % include second image
%   \includegraphics[width=.99\linewidth]{imgs/skeletons/skeleton_two_knees.png}  
%   \captionsetup{justification=centering}
%   \caption{Part\\Knee}
%   \label{subfig:knee}
% \end{subfigure}
% \begin{subfigure}{.10\textwidth}
%   \centering
%   % include second image
%   \includegraphics[width=.99\linewidth]{imgs/skeletons/skeleton_two_feet.png}  
%   \captionsetup{justification=centering}
%   \caption{Part\\Foot}
%   \label{subfig:two_feet}
% \end{subfigure}
% \begin{subfigure}{.10\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=.99\linewidth]{imgs/skeletons/skeleton_left_hand.png}  
%   \captionsetup{justification=centering}
%   \caption{Left\\Hand}
%   \label{subfig:left_hand}
% \end{subfigure}
% \begin{subfigure}{.10\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=.99\linewidth]{imgs/skeletons/skeleton_right_hand.png}  
%   \captionsetup{justification=centering}
%   \caption{Right\\Hand}
%   \label{subfig:right_hand}
% \end{subfigure}
% \caption{Illustrations of different angles. The two sides of an angle are the green dashed lines. }
% \label{fig:RNI_Front}
% \end{figure*}

\section{Angular Graph Networks}
\subsection{Challenges in Using Joint Coordinates}
% Skeleton-based action recognition, compared with the video-based counterpart, has a more compact representation of human poses. Furthermore, skeletons are advantageous over videos in removing the interference of backgrounds. However, 
%When performing two different actions, the positions of joints from two skeletons can be similar, leading to differentiating the two actions challenging. For example, if one uses Kinetic V2 to estimate skeleton joints, a hand will only consist of three joints: a hand tip, a thumb, and a wrist. Utilizing only three joints makes distinguish different gestures tough, such as discern playing a phone from typing on a keyboard. 
Discriminating skeleton actions is quite tough, not least because intra-class differences may be large relative to inter-class. Consider distinguishing typing on a keyboard from operating a phone. Typists may use either touch typing or a hunt-and-peck technique. In terms of motions, the latter is more similar to operating a phone than to touch typing. Indeed, in Kinetic V2 representation, where a hand consists of only a wrist, a thumb and a hand tip, the touch typist may appear almost motionless. However for a given subject there is one fairly reliable discriminator: the keyboard will generally be further away from the body than the phone, and the hands likewise.

However a discriminator that directly uses this difference faces a problem. The distance also depends on the height of the subject: a taller subject will generally have both phone and keyboard at a greater distance from the body center. What is important is the relative distance. While this can, in principle, be learnt, it adds very substantially to the complexity of the learning problem.
%Therefore, in order to let a neural network differentiate two skeletons with similar positions of joints, the network is required to build up the mapping between the relative distances among joints and the action classes. For example, generally two hands are further away from the body center when typing on a keyboard than operating a phone. However, mapping the relative distances among joints to an action is non-trivial, since the changes in distances are not only caused by different actions, but also due to the variations of subjects. For example, a taller person is expected to have a longer arm, and thus his hands will have larger distances to the body center. Therefore, if employing the coordinates of joints to recognize different actions, the networks needs overcoming subject variations, leading to action recognition difficult. 

We require a quantity that can reflect the relative distances among joints, yet is invariant among different subjects: that is, we are concerned with similarity (in the geometric sense) between skeletons, not congruence. 
%Angles are such quantities, since angles maintain invariance given two similar objects, and human skeletons are mutually similar. 
Thus, using angles among joints within a skeleton can resist influences resulting from subject variations. 

In this paper, rather than directly using the angle $\theta$ between three joints, we instead use the quantity $1-\cos{\theta}$ with the property that the angular feature increases monotonically with the angle (for angles between 0 and $\pi$ radians). 

Instead of obtaining angular features in a predefined fashion, is it feasible to assist a network to implicitly learn angular features? Learning angular features is challenging for two reasons. Current state-of-the-art results for skeleton-based action recognition are achieved by graph neural networks. In order to develop angular features among long-range joints, a graph neural network would need to perform multiple stages of message passing and feature aggregating. Recent research \cite{li2018deeper,Zhao2020PairNorm} suggests that performance will be compromised if a graph neural network has too many layers. Moreover the commonly used networks for skeleton-based action recognition, \ie graph neural networks and self-attention networks, model pairwise relationships between joints. Graph networks aggregate neighbor features based on a two-dimensional adjacency matrix, and self-attention models learn new joint features by computing pairwise dot products. Angular features involve three joints, so current mainstream networks are not aligned with the requirements for inferring angles.  

\subsection{Selecting Angles}
Going from order two features (joint-to-joint vectors) to order three (angles between joints) raises the feature complexity of skeleton action recognition from $O(N^2 T D^2)$ to $O(N^3 T D^2)$, where $N$ represents the number of joints within a skeleton, $T$ is the number of frames, and $D$ is the feature dimension. This is likely to be infeasible; so  to reduce computational cost,
%The complexity of $O(N^3)$ is impractical. Thus, 
we manually define sets of angles that are likely to facilitate differentiation of action classes without drastically increasing computational cost. Our selected angles can be classified into four classes, as detailed below. 
%Next, we describe what properties does each class of angles depict, as well as how are the angle sides among the three joints determined. 
\\
\textbf{Local-Bone Angles.} Local-bone angles are the angles shaped by two adjacent bones, as~\autoref{subfig:local_bone} illustrates. This is a third-order extension to the bone representation. Whereas a bone feature relates two joints, an angle feature relates two bones. Specifically, the angular feature for joint $u$ is defined as: 
\begin{align}
    a_{l}(u) = 1 - \frac{ \vec{b}_{uv_1} \cdot \vec{b}_{uv_2} }{ |\vec{b}_{uv_1}| |\vec{b}_{uv_2}| }, 
\end{align}
where $v_1$ and $v_2$ are adjacent joints of $u$, and $\vec{b}_{uv_1}$ and $\vec{b}_{uv_2}$ representing the two bone vectors with joint $u$ as the root. When a joint has more than two bones connecting to it, we pick the most active bone pair instead of using all possible pairs. For example, for the neck joint, we use the two bones connecting to the shoulders, rather than those linking head and belly, since the latter rarely move.  

Local-bone angles promote discrimination between actions where the positions of joints are close together. For example, a person's head and neck are right next to each other, so their coordinates are similar. using the positions of these joints and the bones on the arms to distinguish beteen touching the head or the neck is challenging. However the angles between the fore- and arm arm differ greatly between the two actions, and thus can resolve the confusion. 
\\
\textbf{Center-Oriented Angles.}
Local-bone angles reflect the relative movement of a joint relative to neighbouring joints. Regarding long-range joints, we consider the relative distance between every joint to the center of the body. Specifically, we fix the two joints at the body center, and let the third joint be any other joint within the skeleton. 

Using relative distances to the body center can help discriminate actions whose skeletons are similar. For example in raw joint coordinates, the skeletons for typing on a keyboard and playing with a phone are quite similar. However a person's hands are closer to the body center when operating a phone than a keyboard, so adding the distances from the hands to the human center can help to differentiate the two actions. 

To represent the distances from every joint to the body center, we can either directly calculate such distances as a part of the input feature, generating scale problems, or we can use the angle between the two central joints and the additional joint to reflect the distance in a scale- (i.e. subject-) independent manner. %However, using distances directly will induce intra-subject variances, as explained earlier. In contrast, angles are invariant given two similar skeletons. Thus, we employ the angular features. 

\rim{I'm sorry, I am completely confused by the next three paragraphs. Regarding the angles b and c as shown in figures 3b and 3c, don't we just have $c=\pi-b$? I don't understand the point of this discussion. Skipping the rest of this section pending clarification. I'm also skipping Part-based angles, because it seems to be still under construction. }

\rim{I'm further confused, because at the start of this subsection, we are promised four types of angles, but there seem to only be three (local, center oriented, part-based)?)}

When shaping an angle, we undertake two approaches. First, we connect the joint to the two central joints respectively, as~\autoref{subfig:center_joint} illustrates. This angle expresses the proximity to the body center. In more detail, as the joint moves toward the body center, the angle becomes larger. 
% Formally, we express this center-oriented angle $c_1$ for joint $u$ as follows: 
% \begin{align}
%     a_{c_1}(u) = 1 - \frac{ \vec{b}_{uc_1} \cdot \vec{b}_{uc_2} }{ |\vec{b}_{uc_1}| |\vec{b}_{uc_2}| }, 
% \end{align}
% where $c_1$ and $c_2$ are the two joints in the body center. 

Second, we keep the connection of the two central joint, \ie the skeleton central axis, a constant side of the angle, and link the lower central joint with the third joint, as~\autoref{subfig:center_axis} depicts. Such an angle reflects the distance between the joint to the human central axis. That is, as the joint moves closer to the central axis, the angle becomes smaller. 
% In formula, we express this center-oriented angle $c_2$ for joint $u$ as below: 
% \begin{align}
%     a_{c_2}(u) = 1 - \frac{ \vec{b}_{c_2c_1} \cdot \vec{b}_{c_2 u} }{ |\vec{b}_{c_2c_1}| |\vec{b}_{c_2 u}| }, 
% \end{align}
% where $c_1$ and $c_2$ are the two joints in the body center. 

Furthermore, the angle also indicates the amplitude of motion, where a larger angle implies a more energetic action. Different actions may require distinct strengths, and thus motion amplitudes can assist in action recognition. For instance, the amplitude of hitting other person with something is generally larger than wielding knife towards the other person, although the the skeletons for the two actions look similar. 
\\
% \begin{figure}[ht]
% \centering
% \begin{subfigure}{.20\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=.99\linewidth]{imgs/skeletons/skeleton_left_hand.png}  
%   \caption*{Left-Hand}
%   \label{fig:skeleton_left_hand}
% \end{subfigure}
% \begin{subfigure}{.20\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=.99\linewidth]{imgs/skeletons/skeleton_right_hand.png}  
%   \caption*{Right-Hand}
%   \label{fig:skeleton_right_hand}
% \end{subfigure}
% \caption{}
% \label{fig:RNI_Front}
% \end{figure}

\textbf{Part-Based Angles.}
% This paragraph may needs revision since I may use more angles. 
Within a skeleton, not all joints are of the same importance for undertaking actions. For example, hands perform more actions than other body parts, and thus the joints of hands are expected to produce more distinctive features. In this paper, for the key body parts that engage in more actions, we explicitly calculate the angles relating to them. We consider the key parts as hands, elbows, knees, and feet, corresponding to arms and legs. 

We utilize the angle shaped by a body center joint as the angle root, and two other joints are the two located in the mutually symmetric parts. For example, the two other joints are two elbows. The illustrations of hands, elbows, knees and feet are illustrated as Figure~\ref{subfig:two_hands}-\ref{subfig:two_feet}.  
From these part-based angles, we can implicitly know the sizes of the objects relating to the actions. For example, the angle between the two connections from two hands to the body center indicates the magnitude of the object that a person is holding. The sizes contribute to differentiating actions about objects, such as differentiating cutting nails and playing a phone, as nail cutters are smaller phones.

Since hands involve the most action performance compared with other body parts, we build more detailed angles comprising of hand joints if the skeleton of a hand has more than one joint. For example, Kinetic V2 expresses a hand skeleton with three joints. The illustrations are Figure~\ref{subfig:left_hand}-\ref{subfig:right_hand}. 
Such angles about hands can indirectly depict the gestures. For instance, an angle whose root is a wrist and the other two joints are a hand tip and a thumb can reflect the degree of the hand opening, facilitating discerning between making victory and OK gestures. 



\subsection{Building an Efficient Graph Network.}
% The backbone of our model is a spatial-temporal graph neural network (ST-GCN), including three ST-modules. Following~\cite{liu2020disentangling}, when a GCN aggregates spatial joint representations, different adjacency matrices with distinct neighbor scales are employed to learn multi-level spatial features. Furthermore, Inspired by~\cite{shi2019two}, we consider the adjacency matrix of a skeleton learnable via using a parameterized mask and letting the mask add with the adjacency matrix. As to extracting temporal features, we conduct convolution along the temporal axis. The size of a receptive field is fixed to be 3, while the temporal model applies four different dilations to learn multiscale features.
The design aim for our network architecture is efficiency in both storage and time. This is reflected in two objectives: to use fewer parameters and to minimize running time. Based on these
objectives, we follow two implementation principles. First, to avoid stacking graph convolutional layers, because recent work reveals stacking multiple layers compromises performance, known as oversmoothing. Second, to use $1 \times 1$ convolution kernels, because larger ones introduce more parameters and slow down the operations.

These principles result in the architecture depicted in \autoref{fig:net_architecture}. We follow the architecture of MS-G3D \cite{liu2020disentangling}. 

Its backbone is a spatial-temporal graph convolutional network, alternating spatial aggregation and temporal convolution. In spatial message aggregation, we follow the spirit of~\cite{liu2020disentangling} in creating adjacency matrices with multiple scales, to conduct graph convolutions with different sizes of receptive fields. We thus avoid stacking multiple layers of graph convolution. In temporal convolution, we only convolve toward a single joint through time, ignoring its neighbors, thus reducing the number of parameters and accelerating learning. Inspired by~\cite{shi2019two}, we also introduce a learnable mask for the adjacency matrices, making the graphs more flexible. When feeding data to the network, we concatenate angular representations with those previously used by others (see \autoref{tab:compare_with_sota} for details). 


==> secs/rebuttal.tex <==
We thank all the reviewers for their valuable comments. 

% \textbf{R116: The improvement on NTU60 X-View. } As stated in the paper, our backbone is a modified MSG3D instead of the original one, denoted as \enquote{Baseline}. We compare the performances of this baseline model without and with angular features. As Table~\ref{tab:baseline} shows, the angular features can boost accuracy on NTU60 X-View. 
% % Fusing angular features on DeCoup-GCN can
% % %can or may? Can means it almost certainly will, may just means it might.
% % further improve the SOTA performance. However, it will certainly cost more parameters and run time than our backbone. 

% \noindent
% \textbf{R148: No significant improvement of angular features in Table.4}. Our backbone is a modified version of MSG3D where we have removed the time-consuming part (G3D). It is fair to compare the performances with and without using angular features on our backbone model. As depicted in Table1\&2, the improvement resulting from angular features is substantial, with an maximum of 2.53\% increase. We also include the increases caused by angular features on other datasets in Table\ref{tab:baseline}. If we fuse angular features with other backbones, their accuracy can also further improve. 

\noindent
\textbf{R116, R148: No significant improvement of angular features in Table~4. \& R2: Compatibility with other backbones. } 
(1) \textit{\ul{The effectiveness of angular features should be evaluated on the same backbone}}: As stated in \textcolor{blue}{Sec.~3.2}, our backbone is a modified version of MSG3D, where we remove the time-consuming part (G3D), denoted as \enquote{MSG3D (- G3D)} in \autoref{tab:baseline}. 
It is \textit{fair} to compare the results before and after adding angular features on the same backbone instead of comparing with the SOTA results with different backbones. As depicted in \textcolor{blue}{Table~1\&2} and \autoref{tab:baseline}, the improvement resulting from angular features is substantial, with a maximum of 2.9\% increase. For example, we observe a boost of 0.8\% on NTU60 X-View setting (see \autoref{tab:baseline}).
% (2) \textit{\ul{}}: xxx. 
(2) \textit{\ul{The angular features are independent of the choice of backbones.}}
\ul{Thus, they are compatible with any backbones.}
% As \autoref{tab:baseline} shows, fusing the angular features to \enquote{Baseline} can boost accuracy on NTU60 X-View. Furthermore,
As shown in \autoref{tab:baseline}, concatenating angular features with existing ones can also improve accuracy on new backbones such as MSG3D and Shift-GCN on different settings of two datasets. 

\noindent
\textbf{R2: The angle information may be learned by some models. }
We agree with this.
% that angular features may be learned by a powerful network.
However, as discussed in Sec.~1, such a design is challenging for current GCNs.

\noindent
\textbf{R2: Claiming of our model requiring fewer than 70\% of the parameters and run time conflicts with Table 4. }
As written in Sec.~4.4, we are comparing \enquote{with the existing most-accurate model}, \ie{} MSG3D since it achieves SOTA for the most datasets. When outperforming it, our model requires fewer than 70\% of the parameters and run time. 
% The comparison was explicitly stated to be with the SOTA (i.e. MSG3D), not with shift-GCN. However to guarantee against misreading, we will change the sentence to read "Compared with the existing most-accurate model, MSG3D, AngNet requires fewer..."

\noindent
\textbf{R2: GFLOPs of Shift-GCN is small. }
GFLOPs is not a fair metric to compare Shift-GCN with our backbone for the run time, since \ul{Shift-GCN heavily relies on shifting operations instead of convolutions, which are not counted in GFLOPs}. 
As shown in~\autoref{tab:baseline}, the processing time for Shift-GCN is 50\% more than ours (ours is 10 min and Shift-GCN is 15 min per epoch on GPUs, and 5 min of GPU time is very high). We will include the comparison of run time in the final version. 
% On the same computing system, running only the one compute-intensive program, the processing time for Shift-GCN was 33\% more than ours (10 min vs  Shift-GCN's 15 min per epoch; almost all of that time was GPU time). We will include the GPU time in the final version. 

\noindent
\textbf{R2: Confusing finger-based angular features in Fig.~2. } We cannot properly understand the question because there is no wrist in \textcolor{blue}{Fig.~2(d)}'s angles. We think the reviewer means the elbow.
We use the angular features for the right elbow as an example in \textcolor{blue}{Fig.2~(d)} to show how to calculate the relative angles between left or right fingers with a target joint. 
It is just a single example for visualization. In implementation, we calculate the finger-based angular features for every joint. We will provide more details in the final version.
%I think this misses the reviewer's point: why use angles between _left_ fingers and _right_ elbow. I think a reasonable answer is that this is just for illustration, and using the matching elbows would be too hard to see.

% R2 
% \textcolor{blue}{Angular information has been widely used in previous skeleton action recognition methods based on hand-crafted features. Except introducing third-order features as an input to graph networks, the novelty of the network is limited, which is inspired from MS-G3D.}

% \noindent
% \textbf{R27: No question. }

\noindent
\textbf{R116: Mention previous studies on angle features using non-GCN models. }
We will carefully review past studies that use angles and add them in the related work section.
% We are focusing on GCNs. Previous angle-related non-GCN methods will be included in the final version's related work. 

% \noindent
% \textbf{R116: The improvement on NTU60 X-View. } As stated in the paper, our backbone is a modified MSG3D instead of the original one, denoted as \enquote{Baseline}. We compare the performances of this baseline model without and with angular features. As Table~\ref{tab:baseline} shows, the angular features can boost accuracy on NTU60 X-View. 
% % Fusing angular features on DeCoup-GCN can
% % %can or may? Can means it almost certainly will, may just means it might.
% % further improve the SOTA performance. However, it will certainly cost more parameters and run time than our backbone. 

% \noindent
% \textbf{Limitations of our method}. Our model suffers from the problems caused by the limited number of joints in a skeleton. For example, as shown in the paper, our model cannot discern between `yawn' and `blow nose', which even humans cannot differentiate.
%OK, maybe  you need to add "...cannot differentiate using skeletons without additional information such as RGB video or sound"

\noindent
\textbf{R116: In Table~1\&2, \enquote{Cct/Ens: Jnt+Bon}
% and "Ens: Jnt+Bon" 
would be wrong?}.
% (change this shorter. )
% We have looked into these two tables very carefully again, 
We found no error in these two tables. 
As described in the paper, these are two different ways of combing features. \enquote{Cct: Jnt+Bon} means to use a single model to train the concatenation of joint and bone. \enquote{Ens: Jnt+Bon} means to ensemble two models trained by joints and bones separately. 
% perhaps change "As described in the paper, these are two different ways of combing features." to "Perhaps the reviewer missed that..."

\begin{table}[t]
\centering
% \vspace{-2mm}

\resizebox{0.99\columnwidth}{!}{
\begin{tabular}{l | c | rr | rr | r | r | r}
\toprule
% row 1
%\rowcolor{Gray}
& &
\multicolumn{2}{c| }{\textbf{NTU60}} 
& \multicolumn{2}{c|}{\textbf{NTU120}}
% & \multicolumn{2}{c }{\textbf{Kinetics}}
& \multicolumn{1}{c| }{\textbf{\# Para}}
& & \textbf{Time}
\\
% row 2
\cline{3-6}
%\rowcolor{Gray}
\multirow{-2}{*}{\textbf{Methods}} & \multirow{-2}{*}{\textbf{\# Ens}}
& X-Sub
& X-View
& X-Sub
& X-Set
% & Top-1 & Top-5 
& \multicolumn{1}{c| }{\textbf{(M)}}
& \multirow{-2}{*}{\textbf{GFlops}}
& \multicolumn{1}{c }{\textbf{(Min)}}
\\
\midrule 
\!MSG3D (- G3D) (Jnt) & 1 & 87.2 & 93.7 & 82.4 & 83.0 & 1.44 & 19.4 & 10 \\
% \midrule
Cct: AngNet-JA (Jnt+Ang)  & 1 & 88.7 & 94.5 & 83.2 & 83.7 & 1.46 & 19.6 & 10 \\
\midrule
% MSG3D (Jnt) & 1 & 89.3 & 94.9 & 83.3 & 84.4 & 3.22 & 49.0 & 15 \\
\!MSG3D [Liu et al.] (Jnt) & 1 & 88.2 & 94.6 & 83.3 & 84.4 & 3.22 & 49.0 & 15 \\
Cct: MSG3D (Jnt+Ang) & 1 & 89.8 & 95.5 & 84.8 & 85.6 & 3.42 & 50.4 & 15 \\
\midrule
% Shift-GCN~\cite{} & 1 & 87.8 &  & 80.9 & 83.2 & 0.69 & 2.5 & 15 \\
\!Shift-GCN [Cheng et al.] (Jnt) & 1 & 87.4 & 94.8 & 80.9 & 83.2 & 0.69 & 2.5 & 15 \\
Cct: Shift-GCN (Jnt+Ang) & 1 & 88.0 & 95.3 & 83.8 & 83.9 & 0.70 & 2.5 & 15 \\
% \midrule
% DeCoup-GCN~\cite{} & 1 &  &  &  &  &  &  \\
% DeCoup-GCN (Cct Ang) & 1 &  &  &  &  &  &  \\
\bottomrule
\end{tabular}
}
% IJCAI asks people to put captions below the table. 
\vspace{-2mm}
\caption{
Comparison of accuracy before and after fusing angular features. \enquote{Cct} is concatenation. No ensembling multiple models. 
} 
\vspace{-2mm}
\label{tab:baseline}
\end{table}

\begin{figure}[t]
\centering
\begin{subfigure}{.99\columnwidth}
  \centering
  \includegraphics[width=.99\linewidth]{imgs/Rebuttal/skeleton_82.png}
\end{subfigure}

\begin{subfigure}{.99\columnwidth}
  \centering
  \includegraphics[width=.99\linewidth]{imgs/Rebuttal/RGB_82.png}
\end{subfigure}
\vspace{-2mm}
\caption{An example of  \enquote{fold paper} containing subtle details in hands. The second row is the corresponding RGB frames taken from a different viewpoint. Without Angular features, the action is classified as  \enquote{ball up paper}.}
\label{fig:visual_sample}
\vspace{-1mm}
\end{figure}

\noindent
\textbf{R148: Whether angular features are 2D or 3D? Does it involve the consideration of planes?}. 
As given in Eq.(1), $\vec{b}_{uw_1}$ and $\vec{b}_{uw_2}$ are vectors of relative joint positions in either 2D or 3D % arbitrary dimensions 
(3D for NTU60/NTU120, 2D for Kinetics). Therefore, our angular features are computed in 2D/3D space (2D/3D joint coordinates) depending on the dataset, and \ul{it can be extended to not only a plane (2D space) but also arbitrary dimensions (\ie{} 3D, etc)}.
% the input to Eq.(1) can be of arbitrary dimensions. 
% The output of Eq.(1), \ie{} 
Each individual angular feature $d_a(u)$ is a scalar; however, the input dimension of the network is (\#channels, \#frame, \#joints,  \#subjects), where \#channels denotes the number of concatenated features (joint, bone, and angular information) per joint in each frame. 
% It is unclear what the plane means. 
% If the reviewer means to project the 3D angles to a plane, we don't do this projection since it loses information.

% I think by 3D, the reviewer means the angle as measured in the common plane of the 3 points (assuming they are not collinear). I think this is what you used. I think by 2D, the reviewer means the projection onto a single plane (probably, the plan perpendicalar to the viewing axis). I think the reviewer seems to think 2D would be better, but I think it is better to argue that projection loses information, particularly if the plane of the three points is near parallel to the viewing angle.
%Oh sorry, I missed that you had separated the two questions.

% \noindent
% \textbf{R148: Does Eq.(1) involve the consideration of planes?}.
% \textcolor{red}{We cannot properly understand the question. The angular feature is just a scalar. It is unclear what the plane means. The reviewer may mean to project the angles to a plane. We don't conduct projection since it loses information. }

\noindent 
\textbf{R148: The results of only using the angular features. } 
% We kindly request R148 to check Table 2 in the paper. 
% As presented in Table 2 in the paper, 
% We have already included the results where only angular features are used. 
We have presented the results where only angular features are used in \textcolor{blue}{Table 2}. 
On NTU120 XSub, we achieve 81.97\% with only angular features and 79.83\% with angular velocities respectively. These are comparable with using joint features. 
% I would change " As presented in Table 2 in the paper, we have already included the results where only angular features are used. " to "The reviewer appeats to have missed that the base case in Table 2 is precisely the case he has requested." 

\noindent
\textbf{R148: Evaluation on the balance between computation complex, computation cost and additive accuracy improvement of adding the angular features. } As \autoref{tab:baseline} shows, \ul{additional computational complexity and cost are negligible}. Specifically, adding angular features leads to the \#parameter enlarging from 1.44 to 1.46 ($0.02 \uparrow$) and the run time increasing from 19.4 to 19.6 ($0.02 \uparrow$). In contrast, we achieve significant improvement in accuracy (on average $1.08\% \uparrow$). 

% R5 
\noindent
\textbf{R155: Ablation studies on different angular features. } On NTU120 XSub, we evaluate every type of angular features by fusing each with the joint features.
% On NTU120 XSub:
% with our baseline model using the joint features: 
% Baseline (without angular features)
Baseline is MSG3D (- G3D) (Jnt)
(\textbf{82.4\%}); concatenating local (\textbf{82.9\%}); center-oriented (\textcolor{red}{\textbf{83.2\%}}); pair-based (\textbf{83.0\%}); finger-based (\textbf{83.0\%}) angular features. Center-oriented angles are the most effective ones. 
We will add this ablation study in the final version.

\noindent
\textbf{R155: Visual examples on which samples can be corrected by adding such third-order features. } 
% See ~\autoref{fig:visual_sample}
A visual example is shown in~\autoref{fig:visual_sample}. More examples will be presented finally. 

% \begin{table}[t]
% \centering
% % \vspace{-2mm}
% \caption{caption
% } 

% % \resizebox{0.99\columnwidth}{!}{
% \begin{tabular}{c c c c c c}
% \toprule
% % row 1
% %\rowcolor{Gray}
% \textbf{No Ang} & \textbf{Local} & \textbf{Center} & \textbf{Part} & \textbf{Finger} \\
% \midrule 
% 82.4 & 82.9 & 83.2 & & 83.0 & 83.0 \\

% \bottomrule
% \end{tabular}
% % }
% \label{tab:baseline}
% \end{table}

==> secs/rebuttal_raw.tex <==
% R1
\textcolor{blue}{As stated by the authors, the proposed angular features are compatible with the other competing models, but the authors only use MSG3D as the backbone. This leads to the suspect that the angle information may be able to learn by some models automatically. }
\\\textbf{Answer}: Our angular features are also compatible with other backbones. We have conducted experiments on fusing angular features with Shift-GCN on NTU120. 
Put a table to compare with shift gcn. 
\textcolor{purple}{We use the modified version of MSG3D where we remove the time-consuming part (G3D) to further improve the accuracy}
\textcolor{purple}{at bottom, we write our method is compatible with any baseline models. }

\textcolor{blue}{The paper also claims that its Angular Network (AngNet) requires fewer than 70\% of the parameters and less than 70\% of the run time while achieving better recognition results, but this statement is in conflict with the experimental result in table 4. Specifically, in order to gain the same accuracy with the shift-GCN, the number of parameters and GLOPs of the AngNet are larger.}\\
\textcolor{purple}{shift-gcn does not achieve the best accuracy on all the datasets. write the processing time of shift-gcn is 33\% more than ours (ours is 10 minutes and theirs is 15 minutes per epoch on GPUs). The 5 minutes of GPU time is very high. hand-crafted operations, not a lot of convolution, hence GFLOPs is not representative metric for fair comparison in case of shift-gcn. 
In terms of time, ours is faster. 
}
% mention the page number and part of the sentence, 
% we write the sentence in the paper
% 

1. As stated in the paper, we are comparing with the most accurate model. 
2. The running time of Shift-GCN is 15 minutes per epoch, while ours is 10 minutes. Shift-GCN heavily relies on shifting operation instead of floating-point operation. Thus, GFlops cannot accurately reflect its running time. We will include the comparison of running time in the final version. 

\textcolor{blue}{Meanwhile, the figure of finger-based angular features is confusing in figure 2. Why the feature of the left fingers is the angle between the left fingers and the right wrist? And at the same time, the right fingers’ feature is the angle between the right fingers and the right wrist too?}\\
\textcolor{purple}{we cannot understand the question properly because there is no wrist in figure-based angles of figure 2. then explain the figure 2. 
\\ another explanation: this specific features are for calculating features for elbows. We can also calculate this for wrist. 
}
% it is unclear what the wrist is. if it is the elbow, it is just an single example. in implementation, we take every joint into consider, and calculate the angle of two left figures and the joint. 

% R2 
% \textcolor{blue}{Angular information has been widely used in previous skeleton action recognition methods based on hand-crafted features. Except introducing third-order features as an input to graph networks, the novelty of the network is limited, which is inspired from MS-G3D.}

% R3
\textcolor{blue}{In various past action recognition methods, some methods using the joint angle features have been reported (For example, M.Z.Uddin et al., “Human Activity Recognition Using Body Joint-Angle Features and Hidden Markov Model”, ETRI journal, Vol. 33, No. 4, pp.569-579, 2011.). Since they are not GCN-based methods, the novelty of the proposed method is clear. However, since this paper does not refer to other studies that used joint angle features, it is necessary to mention how joint angle features are used in past studies.
}
\textcolor{purple}{we are focusing on GCN. we will include the previously used cases in the final version. }

\textcolor{blue}{In the recognition performance when "X-View" and "NTU60", the performance improvement by the proposed method was not seen, and the comparison method showed better performance than the proposed method. The reason for this was not explained. }\\
Add a line of baseline results. We are comparing with our baseline model instead of the SOTA methods. If we add angular features in other SOTA methods, the corresponding methods will also improve. 
\textcolor{purple}{as stated in the paper, this is not SOTA ms-g3d, a modified version. what is the modification. what is the baseline accuracy. compare the parameters and time. the number of parameters and run time is higher than our current backbone. DeCoup can also be used as the backbone. however, it will cost more parameters and run time. }

\textcolor{blue}{It is also important to explain the limitations of the method, so it will be necessary to discuss or explain it.}\\
We show even for failing cases, the confidences still improve. 
\textcolor{purple}{we will write a paragraph on limitations for our method. our method inherits from the limitations of existing methods. }

\textcolor{blue}{In Table 1 and Table 2, "Coc: Jnt+Bon" and "Ens: Jnt+Bon" would be wrong.?}\\
In table 1, cct: Jnt+Bon means to use a single model for training the concatenated features of joint and bone. In table 2, ens: Jnt+Bon means to ensemble two models trained by joint and bone representations separately. 
\textcolor{purple}{we have looked into table 1 and 2 very carefully again, we found no problem.  
these are two different ways of combing features. }

% R4
\textcolor{blue}{1. The paper focuses on the Angular Feature Representation for action recognition. Eqn. (1) shows the calculation, but it is not clear the Angular Feature is 2D or 3D? Generally, angular should rely on one base plane, the angle values will be different with different base planes. Does Eqn. (1) involve the consideration of planes?}\\
\textcolor{red}{It depends on whether the coordinates are 2D or 3D. }
\textcolor{purple}{as given in figure 2 there is no plain. the angle we calculate is based on a joint a, 
the angles are relative as shown in figure 2, 
}
\textcolor{purple}{the input to Eqn. (1) can either be 2D or 3D, and the output of the equation is the angular feature, is just a scalar. 
}
% whatever the dimensions are given to the
% given two vectors in a euclidean space, the angle is determined by eq (1). it is unclear what the plain means. 
% projection will lose information, we don't do projection. 

2. \textcolor{blue}{If the Angular Feature could represent human action, how about only using the Angular Feature for action recognition? It is required to add evaluation on the Angular Feature.}
\textcolor{purple}{in table 2, we have already included this results where only angular features are used. we achieve xx with only using angular features. }
We have reported the requested results in the first row of Table 2. 
% performance is comparable to ... 

3. \textcolor{blue}{Did the author evaluate the balance between computation complex, the computation cost and the additive accuracy improvement when adding the Angular Feature for recognition? As Table 4 shows, it seems that there is no significant improvement by adding the Angular Feature.}
Add a baseline. And report the relative \% improvement. 
\textcolor{purple}{we have already considered while constructing the angular features. there is negligible computational complexity and cost. we achieve significant improvement in accuracy. 
it's an modified version of msg3d
}

% R5 
1. there seems no ablation study about feature design: local, part based, finger-based features. I wonder the difference between them. E.g. are finger-based features as effective as others?

2. Can the authors show some visual examples on which samples can be corrected by adding such third-order features.


==> secs/rebuttal_with_bob_comments.tex <==
We thank all the reviewers for their valuable comments. 
\begin{figure}[t]
\centering
\begin{subfigure}{.99\columnwidth}
  \centering
  \includegraphics[width=.99\linewidth]{imgs/Rebuttal/skeleton_82.png}
\end{subfigure}

\begin{subfigure}{.99\columnwidth}
  \centering
  \includegraphics[width=.99\linewidth]{imgs/Rebuttal/RGB_82.png}
\end{subfigure}
\caption{An example of  \enquote{fold paper} containing subtle details in hands. The second row is the corresponding RGB frames taken from a different viewpoint. Without Angular feature, the action is classified as  \enquote{ball up paper}.}
\label{fig:visual_sample}
\vspace{-2mm}
\end{figure}

\begin{table}[t]
\centering
% \vspace{-2mm}
\caption{caption
} 

\resizebox{0.99\columnwidth}{!}{
\begin{tabular}{l | c | rr | rr | r | r | r}
\toprule
% row 1
%\rowcolor{Gray}
& &
\multicolumn{2}{c| }{\textbf{NTU60}} 
& \multicolumn{2}{c|}{\textbf{NTU120}}
% & \multicolumn{2}{c }{\textbf{Kinetics}}
& \multicolumn{1}{c| }{\textbf{\# Para}}
& & \textbf{Time}
\\
% row 2
\cline{3-6}
%\rowcolor{Gray}
\multirow{-2}{*}{\textbf{Methods}} & \multirow{-2}{*}{\textbf{\# Ens}}
& X-Sub
& X-View
& X-Sub
& X-Set
% & Top-1 & Top-5 
& \multicolumn{1}{c| }{\textbf{(M)}}
& \multirow{-2}{*}{\textbf{GFlops}}
& \multicolumn{1}{c }{\textbf{(Min)}}
\\
\midrule 
Baseline (Jnt) & 1 & 87.2 & 93.7 & 82.4 & 83.0 & 1.44 & 19.4 & 10 \\
% \midrule
Cct: AngNet-JA (Jnt+Ang)  & 1 & 88.7 & 94.5 & 83.2 & 83.7 & 1.46 & 19.6 & 10 \\
\midrule
% MSG3D (Jnt) & 1 & 89.3 & 94.9 & 83.3 & 84.4 & 3.22 & 49.0 & 15 \\
MSG3D (Jnt) & 1 & xx & 94.8 & 83.3 & 84.4 & 3.22 & 49.0 & 15 \\
CCT: MSG3D (Jnt+Ang) & 1 & 89.8 & 95.5 & 84.8 & 85.6 & 3.42 & 50.4 & 15 \\
\midrule
% Shift-GCN~\cite{} & 1 & 87.8 &  & 80.9 & 83.2 & 0.69 & 2.5 & 15 \\
Shift-GCN~\cite{} & 1 & 85.7 & yy & 80.9 & 83.2 & 0.69 & 2.5 & 15 \\
CCT: Shift-GCN (Jnt+Ang) & 1 & 88.0 & 95.3 & 83.8 & 83.9 & 0.70 & 2.5 & 15 \\
% \midrule
% DeCoup-GCN~\cite{} & 1 &  &  &  &  &  &  \\
% DeCoup-GCN (Cct Ang) & 1 &  &  &  &  &  &  \\
\bottomrule
\end{tabular}
}
\label{tab:baseline}
\end{table}

\noindent
\textbf{R2: Compatibility with other backbones. } 
The angular features are compatible with any backbones. 
We only reported the results with adding angular features on our modified version of MSG3D where we have removed the time-consuming part (G3D) in the main paper. \textcolor{green}{The results on the other backbones are incorporated into Table~4 of the paper with some reformatting without exceeding the page requirements. }
% It is not only compatible with our modified version of MSG3D where we have removed the time-consuming part (G3D), denoted as \enquote{Baseline}, but also compatible with other backbones. 
% Angular features increase the accuracy from 86.9\% to 87.8\%. \textcolor{orange}{maybe include all the results here} We also fuse angular features with Shift-GCN. The accuracy on NTU120 cross-subject improves from x to x.


\noindent
\textbf{R2: Claiming of our model requiring fewer than 70\% of the parameters run time conflicts Table 4. }
As written in Sec.~4.4, we are comparing with the existing most-accurate model, \ie{} MSG3D since it achieves SOTA for the most datasets. When outperforming it, our model requires fewer than 70\% of the parameters and run time. 
The comparison was explicitly stated to be with the SOTA (i.e. MSG3D), not with shift-GCN. However to guarantee against misreading, we will change the sentence to read "Compared with the existing most-accurate model, MSG3D, AngNet requires fewer..."

\noindent
\textbf{R2: GFLOPs of Shift-GCN is small. }
GFLOPs is not a fair metric to compare Shift-GCN with our model for the run time, since \textcolor{red}{Shift-GCN heavily relies on shifting operations instead of convolutions, which are not counted in GFLOPs}. 

The processing time for Shift-GCN is 33\% more than ours (ours is 10 min and Shift-GCN is 15 min per epoch on GPUs, and 5 min of GPU time is very high). We will include the GPU time in the final version. 
On the same computing system, running only the one compute-intensive program, the processing time for Shift-GCN was 33\% more than ours (10 min vs  Shift-GCN's 15 min per epoch; almost all of that time was GPU time). We will include the GPU time in the final version. 

\noindent
\textbf{R2: Confusing finger-based angular features in Fig.~2. }We cannot properly understand the question because there is no wrist in Fig.2(d). We think the reviewer mean the elbow. It is just a single example for visualization. In implementation, we calculate the figure-based angular features for not only elbow and wrist, but for every joint. 
%I think this misses the reviewer's point: why use angles between _left_ fingers and _right_ elbow. I think a reasonable answer is that this is just for illustration, and using the matching elbows would be too hard to see.

% R2 
% \textcolor{blue}{Angular information has been widely used in previous skeleton action recognition methods based on hand-crafted features. Except introducing third-order features as an input to graph networks, the novelty of the network is limited, which is inspired from MS-G3D.}

\noindent
\textbf{R116: Mention previous studies on angle features using non-GCN models. }
We are focusing on GCNs. However we will include non-GCN comparators in the final version's related work. 

\noindent
\textbf{R116: The improvement on NTU60 X-View. } As stated in the paper, our backbone is a modified MSG3D instead of the original one, denoted as \enquote{Baseline}. We compare the performances of this baseline model without and with angular features. As Table~\ref{tab:baseline} shows, the angular features can boost accuracy on NTU60 X-View. 
% Fusing angular features on DeCoup-GCN can
% %can or may? Can means it almost certainly will, may just means it might.
% further improve the SOTA performance. However, it will certainly cost more parameters and run time than our backbone. 

% \noindent
% \textbf{Limitations of our method}. Our model suffers from the problems caused by the limited number of joints in a skeleton. For example, as shown in the paper, our model cannot discern between `yawn' and `blow nose', which even humans cannot differentiate.
%OK, maybe  you need to add "...cannot differentiate using skeletons without additional information such as RGB video or sound"

\noindent
\textbf{R116: In Table 1 and Table 2, "Coc: Jnt+Bon" and "Ens: Jnt+Bon" would be wrong?}.
% (change this shorter. )
% We have looked into these two tables very carefully again, 
We found no error in these two tables. 
As described in the paper, these are two different ways of combing features. In Table 1, \enquote{cct: Jnt+Bon} means to use a single model for training the concatenated features of joint and bone. In Table 2, \enquote{ens: Jnt+Bon} means to ensemble two models trained by joint and bone representations separately. 
% perhaps change "As described in the paper, these are two different ways of combing features." to "Perhaps the reviewer missed that..."

\noindent
\textbf{R148: Whether angular features are 2D or 3D}. As given in Eq.(1), the input to Eq.(1) can be of arbitrary dimensions. The output of Eq.(1), \ie{} the angular feature, is just a scalar. 
% I think by 3D, the reviewer means the angle as measured in the common plane of the 3 points (assuming they are not collinear). I think this is what you used. I think by 2D, the reviewer means the projection onto a single plane (probably, the plan perpendicalar to the viewing axis). I think the reviewer seems to think 2D would be better, but I think it is better to argue that projection loses information, particularly if the plane of the three points is near parallel to the viewing angle.
%Oh sorry, I missed that you had separated the two questions.

\noindent
\textbf{R148: Does Eq.(1) involve the consideration of planes?}.
\textcolor{red}{We cannot properly understand the question. The angular feature is just a scalar. It is unclear what the plane means. The reviewer may mean to project the angles to a plane. We don't conduct projection since it loses information. }

\noindent 
\textbf{R148: The results for only using the angular features for action recognition. } 
We kindly request R148 to check Table 2 in the paper. 
% As presented in Table 2 in the paper, 
We have already included the results where only angular features are used. 
On NTU120 XSub, we achieve 81.97\% with angular features and 79.83\% with angular velocities respectively. These are comparable with using joint representations. 
% I would change " As presented in Table 2 in the paper, we have already included the results where only angular features are used. " to "The reviewer appeats to have missed that the base case in Table 2 is precisely the case he has requested." 

\noindent
\textbf{R148: Evaluation on the balance between computation complex, the computation cost and the additive accuracy improvement of adding the angular features. } As Table~\ref{tab:baseline} shows, the additional computational complexity and cost are negligible. Specifically, adding angular features leads to the number of parameters enlarging from 1.44 to 1.46 ($0.02 \uparrow$) and the run time increasing from 19.4 to 19.6 ($0.02 \uparrow$). In contrast, we achieve significant improvement in accuracy (averagely $1.08\% \uparrow$). 
%This will be mentioned in the final version.

\noindent
\textbf{R148: No significant improvement of angular features in Table.4}. Our backbone is a modified version of MSG3D where we have removed the time-consuming part (G3D). It is fair to compare the performances with and without using angular features on our backbone model. As depicted in Table1\&2, the improvement resulting from angular features is substantial, with an maximum of 2.53\% increase. We also include the increases caused by angular features on other datasets in Table\ref{tab:baseline}. If we fuse angular features with other backbones, their accuracy can also further improve. 

% R5 
\noindent
\textbf{R155: Ablation studies about using different kinds of angular features. } We will include in the final version. 
%I think this could reasonably go in the supplementary materials

\noindent
\textbf{R155: Visual examples on which samples can be corrected by adding such third-order features. } A visual example is shown in~\autoref{fig:visual_sample}. More examples will be presented in the final version. 


%Overall, you are promising to add quite a lot of material to the paper. I don't understand how it can fit (the paper is very tight). Does the conference support supplementary material? It might be better to add some of these extra materials as supplementaries if that is possible.

% Yes. We can add them as supplementary material.

% Yep, I think it's more a matter of saying quite clearly which will go as supplementary material, and which is either already in the paper (we will amend to make it clearer), or is sufficiently small that we can just add it to the paper and rearrange. If we're going to do that, we might  have to also identify some less important content in the paper that we will move to the supplementary.

\begin{table}[t]
\centering
% \vspace{-2mm}
\caption{caption
} 

\resizebox{0.99\columnwidth}{!}{
\begin{tabular}{l | c | rr | rr | r | r | r}
\toprule
% row 1
%\rowcolor{Gray}
& &
\multicolumn{2}{c| }{\textbf{NTU60}} 
& \multicolumn{2}{c|}{\textbf{NTU120}}
% & \multicolumn{2}{c }{\textbf{Kinetics}}
& \multicolumn{1}{c| }{\textbf{\# Para}}
& & \textbf{Time}
\\
% row 2
\cline{3-6}
%\rowcolor{Gray}
\multirow{-2}{*}{\textbf{Methods}} & \multirow{-2}{*}{\textbf{\# Ens}}
& X-Sub
& X-View
& X-Sub
& X-Set
% & Top-1 & Top-5 
& \multicolumn{1}{c| }{\textbf{(M)}}
& \multirow{-2}{*}{\textbf{GFlops}}
& \multicolumn{1}{c }{\textbf{(Min)}}
\\
\midrule 
Baseline (Jnt) & 1 & 87.2 & 93.7 & 82.4 & 83.0 & 1.44 & 19.4 & 10 \\
% \midrule
Cct: AngNet-JA (Jnt+Ang)  & 1 & 88.7 & 94.5 & 83.2 & 83.7 & 1.46 & 19.6 & 10 \\
\midrule
% MSG3D (Jnt) & 1 & 89.3 & 94.9 & 83.3 & 84.4 & 3.22 & 49.0 & 15 \\
MSG3D (Jnt) & 1 & xx & 94.8 & 83.3 & 84.4 & 3.22 & 49.0 & 15 \\
CCT: MSG3D (Jnt+Ang) & 1 & 89.8 & 95.5 & 84.8 & 85.6 & 3.42 & 50.4 & 15 \\
\midrule
% Shift-GCN~\cite{} & 1 & 87.8 &  & 80.9 & 83.2 & 0.69 & 2.5 & 15 \\
Shift-GCN~\cite{} & 1 & 85.7 & yy & 80.9 & 83.2 & 0.69 & 2.5 & 15 \\
CCT: Shift-GCN (Jnt+Ang) & 1 & 88.0 & 95.3 & 83.8 & 83.9 & 0.70 & 2.5 & 15 \\
% \midrule
% DeCoup-GCN~\cite{} & 1 &  &  &  &  &  &  \\
% DeCoup-GCN (Cct Ang) & 1 &  &  &  &  &  &  \\
\bottomrule
\end{tabular}
}
\label{tab:baseline}
\end{table}

==> secs/related_work_backup.tex <==
\section{Related Work}

% {\bf AR using RGB and optical flow videos.} 
% AR has seen significant advances in terms of the overall performance in recent years. Most existing methods~\cite{ji_2013_tpami} treat this problem as a generic classification problem, and the only difference from ImageNet is that the input is now a video sequence, thus numerous efforts have been devoted to leveraging the temporal information. Unlike objects in the ImageNet, which are usually centered and occupy the majority of pixels, human activities are more complex concepts in terms of many factor such as body movement, temporal structure, and human-object interaction.

% The complex nature of human activities indicates that rough modeling of the visual or temporal features results in the confusion between many action classes that share similar factors. A common example of rough modeling is the widely used classifier head of a global average pooling and one linear classifier in AR models, a setup typical of the image object recognition models on ImageNet. For fine-grained AR, confused classes can only be distinguished by further capturing the fine-grained patterns.

{\bf AR using RGB and optical flow videos.}
The 3D CNNs is designed to capture the spatio-temporal features as the 3D convolution is able to represent the spatial features as well as the temporal features together benefiting from the extended temporal dimension. By stacking the 3D convolutions, the 3D CNN can capture the long-term temporal relationship but it also introduce the computational cost a lot. With the help of pre-training on large-scale video datasets such as Kinetics, the 3D CNN-based methods have achieved superior performance compared to 2D CNN-based methods. However, many methods still integrate an independent optical flow stream to further improve the performance with the motion information. Thus, these two information are complementary to each other in AR. Although these methods achieve good performance, they also introduce a large number of parameters that results in computation burdens. Some research work~\cite{Xie_2018_ECCV} attempt to reduce the cost by decomposing a 3D convolutional kernel into spatial and temporal part separately. 

However, these types of methods suffer from two main limitations: (i) these methods require the pre-computation of optical flow, which is expensive; (ii) the learned features and final prediction from multiple streams are fused simply using weighted or average sum, making it inferior to temporal relationship modeling. Almost all of these works maintain the same last layers of the network, which consist of a global average pooling followed by a fully connected layer.

{\bf AR using skeletons.} Different from RGB video based AR methods, which mainly focus on modeling the spatial and temporal representations from RGB frames and/or optical flow videos, skeleton-based AR methods do not suffer from limitations such as background clutter, illumination changes, and appearance variation. 3D skeleton data represents the body structure with a set of 3D coordinates of human body joints, and such robust representation allows us to model discriminative temporal characteristics of human actions. Thanks to the Microsoft Kinect and advanced human pose estimation algorithms~\cite{Cao_2017_CVPR} that make it much easier to get the skeleton data.

% Graph-based model is one of the state-of-the-art methods for skeleton-based AR due to its effective representation for the graph structure data. The current existing graph-based model mainly falls into two categories: (i) graph neural network (GNN), which is a combination of graph and recurrent neural network; (ii) graph convolutional network (GCN), which generalizes convolutional neural networks to graph. There are two types of GCNs, spectral GCNs and spatial GCNs. Spectral GCNs transform graph signals on graph spectral domains and then apply spectral filters on spectral domain. For example, in~\cite{kipf2017semi}, spectral GCN is used for semi-supervised classification on graph-structured data. For spatial GCNs, the convolution operation is applied to compute a new feature vector for each node using its neighborhood information. For example, a spatial temporal graph convolutional network (ST-GCN) is proposed in~\cite{yan2018spatial} for AR. Each spatial temporal graph convolutional layer constructs spatial characteristics with a graph convolutional operator, and models the temporal dynamics with a convolutional operator. 

The earliest attempts of skeleton-based AR often encode all the human body joint coordinates in each frame to a feature vector for pattern learning~\cite{lei_tip2019}. These models rarely explore the internal dependencies between body joints, which results in missing abundant/rich actional information. To capture the joint dependencies, recent methods construct a skeleton graph whose vertices are joints and edges are bones, and apply the GCN to extract the correlected features. The ST-GCN~\cite{yan2018spatial} is further developed to simultaneously learn spatial and temporal features. Although ST-GCN extracts the features of joints directly connected via bones, structurally distant joints, which may cover key patterns of actions, are largely ignored. For example, while walking, hands and feet are strongly correlated. While ST-GCN tries to aggregrate the wider-range features with hierarchical GCNs, node features might be weaken during the long fusion.

..........

{\bf --- Lei up to here ---}

The pioneering work for skeleton-based action recognition focuses on manually designing a function to map a skeleton video to a representation, \st{followed by employing a classifier taking the representations as the input.}\SA{which is then forward to a classifier.} \st{The learning process of these}\SA{The above mentioned} early approaches \st{is}\SA{are} not \SA{trained} in an end-to-end fashion, and thus the classification accuracy is unsatisfactory\SA{comment: not necessary, it can be accurate but not efficient}. Later, convolutional neural networks (CNNs) have been introduced in tackling the problem and \st{receive}\SA{achieve an} improvement in recognizing capability. However, CNNs are designed for grid-based data\st{; therefore, CNNs} \SA{and} are not suitable for graph data since they cannot leverage a graph's topology. Subsequently, graph neural networks (GNNs) emerge and are adopted in identifying skeleton-based actions, achieving \SA{a} substantial increase in \st{accuracy}\SA{performance}. Hence, we primarily \SA{focus on} \st{review} GNN-based models. 

\st{For GNN-based models,a} \SA{A} skeleton is treated as a graph, where joints are nodes and bones are edges \SA{for GNN-based models}. An early application of GNN is ST-GCN~\SA{(citation required)}, using graph convolution to aggregate joint features spatially\st{,} and convolving consecutive frames along the temporal axis. Subsequently, AS-GCN~\SA{(citation required)} is proposed to further improve the spatial feature aggregation via \st{making} the \SA{learnable} adjacency matrix \st{learnable,} instead of utilizing the skeleton as a fixed graph. Afterward, AGC-LSTM~\SA{(citation required)} \st{arises to} learn\SA{s} long-range temporal dependencies\st{. The backbone of AGC-LSTM is a LSTM, yet change}\SA{using LSTM as a backbone and changing} every gate operation from the original fully connected layer to a graph convolution layer, making the best of the skeleton's topology.  

Concurrently, 2s-AGCN~\SA{(citation required, also check whether the name is correct or not)} is presented\st{. It has} \SA{as having} two major contributions. First\SA{ly}, it applies a learnable residual mask to the adjacency matrix of the graph convolution, making the skeleton's topology more flexible. Second\SA{ly}, it proposes a second-order feature, the subtraction between the coordinates of two adjacent joints, to act as the bone information. Via ensembling\SA{,} two models trained with the original feature\SA{s} and the \st{new} second-order feature\SA{s}, the classification accuracy can be improved substantially. \st{Then,} \SA{M}ore novel graph convolution techniques have been \st{conceived or introduced}\SA{published} in recognizing skeleton-based actions, such as SGN, Shift-GCN $\&$ \st{and} DeCoup-GCN, utilizing self-attention, shift convolution and graph-based dropout, \etc\st{, respectively.}. \SA{Recently, MS-G3D~\SA{(citation required)} achieved the current state-of-the-art results} \st{The current state-of-the-art results are achieved by MS-G3D.} by not limiting message passing and aggregation to within a single frame, but instead proposing graph 3D convolution extended to a window of consecutive frames, boosting the \st{recognizing} \SA{recognition} accuracy significantly. However, \SA{the} experiment reveals \SA{experiments reveal} a large running time \SA{for} the 3D convolution\SA{s}. 

\SA{Comment: Write a few lines about our methods for comparison purposes.}

\SA{I am here}


==> secs/related_work_old.tex <==
\section{Related Work}
We review the key research in skeleton-based action recognition.
% \rim{unnecessary: in an narrative fashion.} 
We classify them into three groups according to their backbone models. 
\\
\textbf{Hand-Crafted Feature Based.} When extracting features, the early skeleton-based systems did not require training. Instead, they used human-designed functions to process the spatial and temporal features and map the video to a point or curve in a predefined space. 
For example,~\cite{vemulapalli2014human} transform a video to a curve on a manifold, while~\cite{hussein2013human} convert the frames to a covariance matrix. Despite their solid mathematical support, the classification accuracy of these methods based on hand-crafted features was unsatisfactory.
\\
\textbf{CNN Based.} Subsequent research used convolutional neural networks (CNNs) to conduction classification, relying on the power of CNNs for feature extraction. However CNNs cannot leverage the graph structure of skeletons. 
\\
\textbf{GNN Based.} More recently, graph neural networks have been employed in recognizing skeleton actions. These graphs make use of the connections among different body parts to gain greater classification accuracy. The initial versions~\cite{yan2018spatial} used first-order features alone, then~\cite{shi2019two} proposed using the vector difference between the coordinates of adjacent joints as second-order features. Later work introduced recurrent networks into GNNs to better capture the temporal relationships~\cite{si2019attention}.  

==> secs/tables/complete_action_table_static.tex <==
% \begin{table*}[t]
% \caption{A comparison of with/without angular features on the most confusing actions that may share similar motion trajectories.
% % The most confusing actions predicted by a network trained with joint features only, and the performance from a network trained with combined joint and angular features. 
% The `Action' column shows the ground truth labels, and the `Similar Action' column shows the predictions from the model (with/without angular features).
% % Similar action indicates the most frequently misclassified action by the corresponding classifier. 
% %Acc stands for the accuracy and Acc$\uparrow$ denotes the %an absolute amount of 
% %improvement. %in accuracy. 
% %Jnt and ang represent joint and angular features, respectively. 
% The similar actions highlighted in orange demonstrate the change of predictions after employing angular features. 
% % The accuracy improvements highlighted in red (Acc$\uparrow$ $\geq$ 10\%) are obtained from using our angular features.
% The accuracy improvements highlighted in red are the substantially increased ones (Acc$\uparrow$ $\geq$ 10\%) due to using our angular features.
% } 
% \centering
% % \vspace{-2mm}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|rc|rrc}
% \toprule 
% %\rowcolor{Gray}
%  & \multicolumn{2}{c|}{\textbf{Joint}} & \multicolumn{3}{c}{\textbf{Concatenation: Joint + Angular}} \\
% \cline{2-3}\cline{4-6}
% %\rowcolor{Gray}
% \multirow{-2}{*}{\textbf{Action}} & Acc (\%) & Similar Action & Acc (\%) & Acc$\uparrow$ (\%) & Similar Action \\ 
% \midrule 
% \rowcolor{Gray!30}
% staple book & 31.00 & cutting paper (use scissors) & 40.80 & 9.80 & cutting paper (use scissors) \\
% make victory sign & 35.13 & make ok sign & 61.39 & \textcolor{red}{\textbf{26.26}} &
% make ok sign \\ 
% \rowcolor{Gray!30}
% make ok sign & 40.86 & make victory sign & 66.78 & \textcolor{red}{\textbf{25.92}} & make victory sign \\
% counting money & 51.05 & play magic cube & 56.14 & 5.09 & play magic cube \\
% \rowcolor{Gray!30}
% writing & 53.30 & typing on a keyboard & 61.20 & 7.90 & typing on a keyboard \\ 
% reading & 55.67 & writing & 63.73 & 8.06 & writing \\
% \rowcolor{Gray!30}
% blow nose & 59.13 & \textcolor{orange}{\textbf{hush (quite)}} & 65.21 & 6.08 & \textcolor{orange}{\textbf{yawn}} \\ 
% hit other person w sth & 60.00 & wield knife toward other person & 68.17 & 8.17 & wield knife toward other person \\
% \rowcolor{Gray!30}
% cutting paper & 62.65 & staple book & 68.76 & 6.11 & staple book \\ 
% thumb up & 64.00 & \textcolor{orange}{\textbf{make victory sign}} & 78.78 & \textcolor{red}{\textbf{14.78}} & \textcolor{orange}{\textbf{thumb down}} \\
% \rowcolor{Gray!30}
% cutting nails & 64.17 & playing w phone/tablet & 67.83 & 3.66 & playing w phone/tablet \\ 
% snapping fingers & 64.28 & \textcolor{orange}{\textbf{thumb up}} & 72.12 & 7.84 & \textcolor{orange}{\textbf{make victory sign}} \\
% \rowcolor{Gray!30}
% fold paper & 64.32 & \textcolor{orange}{\textbf{ball up paper}} & 76.00 & \textcolor{red}{\textbf{11.68}} & \textcolor{orange}{\textbf{counting money}} \\ 
% playing w phone/tablet & 65.91 & \textcolor{orange}{\textbf{play magic cube}} & 68.09 & 2.18 & \textcolor{orange}{\textbf{typing on a keyboard}} \\ 
% \rowcolor{Gray!30}
% yawn & 66.18 & \textcolor{orange}{\textbf{hush (quiet)}} & 70.26 & 4.08 & \textcolor{orange}{\textbf{blow nose}} \\ 
% wield knife toward other person & 66.84 & hit other person w sth & 68.14 & 1.30 & hit other person w sth \\ 
% \rowcolor{Gray!30}
% typing on a keyboard & 68.11 & writing & 71.27 & 3.16 & writing \\ 
% open a box & 68.36 & reading & 80.31 & \textcolor{red}{\textbf{11.95}} & reading \\
% \rowcolor{Gray!30}
% sneeze/cough & 68.84 & touch head (headache) & 70.65 & 1.81 & touch head (headache) \\
% \bottomrule 
% \end{tabular}
% }
% \label{table:confusion}
% \end{table*}

\begin{table*}[t]
\centering
% \vspace{-2mm}
\caption{Static: First Half. }
\resizebox{\textwidth}{!}{
\begin{tabular}{l|rc|rrc}
\toprule 
%\rowcolor{Gray}
 & \multicolumn{2}{c|}{\textbf{Joint}} & \multicolumn{3}{c}{\textbf{Concatenation: Joint + Angular}} \\
\cline{2-3}\cline{4-6}
%\rowcolor{Gray}
\multirow{-2}{*}{\textbf{Action}} & Acc (\%) & Similar Action & Acc (\%) & Acc$\uparrow$ (\%) & Similar Action \\ 
\midrule 
% \rowcolor{Gray!30}
make victory sign & 18.48 & thumb up   & 53.04 & 34.57 & make ok sign   \\
staple book & 26.67 & staple book   & 37.13 & 10.46 & cutting paper (using scissors)   \\
writing & 28.41 & typing on a keyboard   & 48.90 & 20.49 & typing on a keyboard   \\
counting money & 48.47 & play magic cube   & 52.98 & 4.51 & play magic cube   \\
playing with phone/tablet & 48.82 & play magic cube   & 59.64 & 10.82 & writing   \\
wield knife towards other person & 49.52 & hit other person with something   & 62.50 & 12.98 & hit other person with something   \\
% make ok sign & 54.48 & make victory sign   & 48.52 & -5.96 & make victory sign   \\
blow nose & 55.35 & yawn   & 59.65 & 4.30 & yawn   \\
fold paper & 56.57 & ball up paper   & 62.78 & 6.22 & counting money   \\
reading & 58.34 & cutting paper (using scissors)   & 64.10 & 5.76 & writing   \\
thumb up & 58.65 & make victory sign   & 72.35 & 13.70 & make victory sign   \\
yawn & 59.00 & hush (quite)   & 67.65 & 8.65 & hush (quite)   \\
snapping fingers & 59.10 & shake fist   & 65.51 & 6.40 & make victory sign   \\
open a box & 59.98 & fold paper   & 71.60 & 11.63 & open bottle   \\
% play magic cube & 62.81 & counting money   & 59.97 & -2.85 & playing with phone/tablet   \\
% cutting nails & 63.32 & playing with phone/tablet   & 63.09 & -0.23 & playing with phone/tablet   \\
pointing to something with finger & 64.58 & taking a selfie   & 79.71 & 15.13 & taking a selfie   \\
sneeze/cough & 64.58 & touch head (headache)   & 71.74 & 7.16 & touch head (headache)   \\
apply cream on hand back & 67.82 & open bottle   & 72.30 & 4.48 & rub two hands together   \\
cutting paper (using scissors) & 68.28 & staple book   & 70.16 & 1.87 & staple book   \\
typing on a keyboard & 68.45 & cutting paper (using scissors)   & 69.09 & 0.64 & writing   \\
% hit other person with something & 69.09 & wield knife towards other person   & 62.26 & -6.83 & wield knife towards other person   \\
hush (quite) & 69.16 & yawn   & 72.08 & 2.92 & yawn   \\
ball up paper & 69.26 & fold paper   & 71.30 & 2.04 & fold paper   \\
eat meal/snack" & 69.55 & brushing teeth   & 71.27 & 1.73 & brushing teeth   \\
wear a shoe & 70.43 & take off a shoe   & 85.35 & 14.92 & take off a shoe   \\
% shoot at other person with a gun & 70.83 & take a photo of other person   & 70.09 & -0.74 & point finger at the other person   \\
take off a shoe & 70.90 & wear a shoe   & 81.75 & 10.85 & wear a shoe   \\
punching/slapping other person & 72.36 & hit other person with something   & 82.85 & 10.49 & hit other person with something   \\
open bottle & 73.17 & play magic cube   & 73.82 & 0.65 & open a box   \\
put something into a bag & 73.26 & take something out of a bag   & 79.13 & 5.87 & take something out of a bag   \\
shake fist & 74.69 & hand waving   & 76.39 & 1.69 & snapping fingers   \\
touch head (headache) & 75.45 & drink water   & 82.25 & 6.80 & touch neck (neckache)   \\
thumb down & 75.52 & thumb up   & 80.87 & 5.35 & pointing to something with finger   \\
sniff (smell) & 76.04 & blow nose   & 81.04 & 5.00 & blow nose   \\
make a phone call/answer phone & 80.09 & reading   & 87.64 & 7.55 & playing with phone/tablet   \\
% flick hair & 80.39 & blow nose   & 80.00 & -0.39 & brushing hair   \\
% throw up cap/hat & 80.50 & shoot at the basket   & 78.01 & -2.49 & toss a coin   \\
apply cream on face & 80.71 & wipe face   & 83.10 & 2.39 & wipe face   \\
rub two hands together & 80.88 & clapping   & 82.61 & 1.72 & apply cream on hand back   \\
touch neck (neckache) & 80.88 & drink water   & 87.32 & 6.43 & flick hair   \\
nausea or vomiting condition & 81.18 & sneeze/cough   & 84.73 & 3.55 & touch chest (stomachache/heart pain)   \\
% shoot at the basket & 81.34 & throw   & 80.24 & -1.10 & throw   \\
drink water & 81.48 & brushing teeth   & 83.94 & 2.46 & brushing teeth   \\
move heavy objects & 81.57 & carry something with other person   & 86.09 & 4.52 & carry something with other person   \\
take something out of a bag & 81.64 & put something into a bag   & 84.90 & 3.26 & put something into a bag   \\
brushing teeth & 81.78 & drink water   & 87.55 & 5.76 & touch head (headache)   \\
drop & 81.91 & staple book   & 85.82 & 3.91 & tear up paper   \\
put the palms together & 81.97 & cross hands in front (say stop)   & 92.75 & 10.78 & sniff (smell)   \\
point finger at the other person & 81.97 & pat on back of other person   & 88.77 & 6.80 & pat on back of other person   \\
use a fan (with hand or paper)/feeling warm & 82.27 & hand waving   & 89.82 & 7.55 & shake fist   \\
check time (from watch) & 82.33 & open bottle   & 90.58 & 8.25 & put the palms together   \\
% clapping & 82.52 & rub two hands together   & 81.69 & -0.83 & rub two hands together   \\
support somebody with hand & 82.65 & follow other person   & 88.70 & 6.04 & knock over other person (hit with body)   \\
take off headphone & 82.92 & take off glasses   & 86.40 & 3.47 & take off glasses   \\
tennis bat swing & 83.15 & throw up cap/hat   & 83.45 & 0.30 & throw up cap/hat   \\
take off glasses & 83.67 & take off headphone   & 93.07 & 9.39 & take off headphone   \\
knock over other person (hit with body) & 83.72 & whisper in other person’s ear   & 88.89 & 5.17 & whisper in other person’s ear   \\
wipe face & 83.78 & brushing hair   & 87.68 & 3.90 & brushing hair   \\
reach into pocket & 84.04 & touch back (backache)   & 85.40 & 1.36 & typing on a keyboard   \\
\bottomrule 
\end{tabular}
}
\label{table:static_complete_action_imp_1}
\end{table*}

\begin{table*}[t]
% Second Half 
\caption{Static: Second Half. }
\resizebox{\textwidth}{!}{
\begin{tabular}{l|rc|rrc}
\toprule 
%\rowcolor{Gray}
 & \multicolumn{2}{c|}{\textbf{Joint}} & \multicolumn{3}{c}{\textbf{Concatenation: Joint + Angular}} \\
\cline{2-3}\cline{4-6}
%\rowcolor{Gray}
\multirow{-2}{*}{\textbf{Action}} & Acc (\%) & Similar Action & Acc (\%) & Acc$\uparrow$ (\%) & Similar Action \\ 
\midrule 
% \rowcolor{Gray!30}
put on headphone & 84.20 & wear on glasses   & 87.52 & 3.32 & take off headphone   \\
throw & 84.82 & wear jacket   & 91.27 & 6.45 & stretch oneself   \\
side kick & 84.89 & kicking something   & 90.77 & 5.88 & kicking something   \\
tear up paper & 84.98 & fold paper   & 88.19 & 3.21 & wear jacket   \\
wear on glasses & 85.08 & drink water   & 88.28 & 3.20 & eat meal/snack"   \\
nod head/bow & 85.23 & nausea or vomiting condition   & 94.93 & 9.70 & nausea or vomiting condition   \\
kicking other person & 85.59 & step on foot   & 91.30 & 5.71 & punching/slapping other person   \\
% grab other person’s stuff & 85.78 & hit other person with something   & 85.57 & -0.22 & touch other person's pocket   \\
touch chest (stomachache/heart pain) & 85.96 & touch back (backache)   & 91.30 & 5.35 & touch back (backache)   \\
toss a coin & 86.09 & throw up cap/hat   & 89.01 & 2.92 & make victory sign   \\
exchange things with other person & 86.48 & giving something to other person   & 89.04 & 2.57 & giving something to other person   \\
step on foot & 86.65 & kicking other person   & 89.39 & 2.74 & kicking other person   \\
cross toe touch & 86.80 & move heavy objects   & 89.90 & 3.09 & move heavy objects   \\
brushing hair & 86.91 & wipe face   & 88.64 & 1.73 & touch head (headache)   \\
taking a selfie & 87.04 & reading   & 90.22 & 3.17 & pointing to something with finger   \\
put on bag & 87.35 & take something out of a bag   & 93.91 & 6.57 & wear jacket   \\
take off bag & 87.72 & tennis bat swing   & 92.36 & 4.65 & take off jacket   \\
whisper in other person’s ear & 87.87 & knock over other person (hit with body)   & 88.87 & 1.00 & knock over other person (hit with body)   \\
% giving something to other person & 88.49 & exchange things with other person   & 87.68 & -0.81 & exchange things with other person   \\
cross arms & 88.74 & cross hands in front (say stop)   & 94.09 & 5.35 & put the palms together   \\
stretch oneself & 88.93 & hands up (both hands)   & 93.06 & 4.13 & hands up (both hands)   \\
cheer up & 89.15 & hand waving   & 90.51 & 1.36 & use a fan (with hand or paper)/feeling warm   \\
put on a hat/cap & 89.44 & wear on glasses   & 94.85 & 5.41 & wear on glasses   \\
salute & 89.58 & shake head   & 92.03 & 2.45 & shake head   \\
hand waving & 89.88 & use a fan (with hand or paper)/feeling warm   & 90.15 & 0.27 & shake fist   \\
% pat on back of other person & 90.30 & point finger at the other person   & 88.77 & -1.54 & point finger at the other person   \\
take a photo of other person & 90.32 & shoot at other person with a gun   & 94.27 & 3.95 & shoot at other person with a gun   \\
hands up (both hands) & 90.81 & stretch oneself   & 94.25 & 3.44 & stretch oneself   \\
take off a hat/cap & 90.94 & throw up cap/hat   & 96.70 & 5.76 & apply cream on face   \\
juggling table tennis balls & 91.15 & toss a coin   & 95.81 & 4.66 & snapping fingers   \\
falling & 91.36 & move heavy objects   & 93.82 & 2.45 & staggering   \\
touch other person's pocket & 91.36 & giving something to other person   & 94.91 & 3.55 & pat on back of other person   \\
touch back (backache) & 91.39 & touch chest (stomachache/heart pain)   & 94.20 & 2.81 & touch chest (stomachache/heart pain)   \\
sitting down & 91.67 & falling   & 94.51 & 2.83 & kicking something   \\
standing up (from sitting position) & 91.67 & take off a shoe   & 95.97 & 4.30 & nausea or vomiting condition   \\
shake head & 91.73 & touch back (backache)   & 92.00 & 0.27 & make victory sign   \\
staggering & 91.75 & walking apart from each other   & 98.91 & 7.16 & follow other person   \\
butt kicks (kick backward) & 91.86 & side kick   & 94.43 & 2.57 & side kick   \\
% pickup & 92.45 & take off a shoe   & 92.00 & -0.45 & take off a shoe   \\
squat down & 92.73 & sitting down   & 96.86 & 4.14 & falling   \\
cross hands in front (say stop) & 92.84 & taking a selfie   & 93.12 & 0.28 & put the palms together   \\
bounce ball & 92.86 & running on the spot   & 94.21 & 1.35 & finger-guessing game (playing rock-paper-scissors)   \\
finger-guessing game (playing rock-paper-scissors) & 92.92 & shake fist   & 94.97 & 2.04 & shake fist   \\
kicking something & 93.20 & side kick   & 94.20 & 1.00 & staggering   \\
hopping (one foot jumping) & 93.55 & staggering   & 96.00 & 2.45 & kicking something   \\
take off jacket & 93.93 & tear up paper   & 96.38 & 2.45 & wear jacket   \\
wear jacket & 94.64 & tear up paper   & 98.91 & 4.27 & put on bag   \\
running on the spot & 95.17 & hopping (one foot jumping)   & 97.39 & 2.22 & butt kicks (kick backward)   \\
high-five & 95.18 & hit other person with something   & 97.05 & 1.87 & giving something to other person   \\
% carry something with other person & 95.18 & move heavy objects   & 93.58 & -1.60 & support somebody with hand   \\
walking apart from each other & 95.38 & walking towards each other   & 96.74 & 1.36 & walking towards each other   \\
arm swings & 95.52 & arm circles   & 98.61 & 3.09 & arm circles   \\
pushing other person & 95.74 & hugging other person   & 96.01 & 0.28 & walking apart from each other   \\
% handshaking & 95.74 & shake head   & 95.29 & -0.45 & giving something to other person   \\
follow other person & 95.88 & walking apart from each other   & 96.01 & 0.13 & walking apart from each other   \\
arm circles & 96.22 & stretch oneself   & 98.96 & 2.74 & stretch oneself   \\
cheers and drink & 96.22 & take a photo of other person   & 97.57 & 1.35 & drink water   \\
hugging other person & 96.45 & falling   & 97.81 & 1.36 & falling   \\
jump up & 96.83 & running on the spot   & 98.19 & 1.36 & kicking something   \\
walking towards each other & 97.17 & follow other person   & 99.27 & 2.10 & staggering   \\
\bottomrule 
\end{tabular}
}
\label{table:static_complete_action_imp_2}
\end{table*}

% % Velocity 

\begin{table*}[t]
\centering
% \vspace{-2mm}
\caption{Velocity: First Half. }
\resizebox{\textwidth}{!}{
\begin{tabular}{l|rc|rrc}
\toprule 
%\rowcolor{Gray}
 & \multicolumn{2}{c|}{\textbf{Joint}} & \multicolumn{3}{c}{\textbf{Concatenation: Joint + Angular}} \\
\cline{2-3}\cline{4-6}
%\rowcolor{Gray}
\multirow{-2}{*}{\textbf{Action}} & Acc (\%) & Similar Action & Acc (\%) & Acc$\uparrow$ (\%) & Similar Action \\ 
\midrule 
% \rowcolor{Gray!30} 
make ok sign & 27.17 & make ok sign   & 46.78 & 19.61 & make victory sign   \\
cutting paper (using scissors) & 27.27 & staple book   & 60.38 & 33.11 & staple book   \\
staple book & 30.17 & cutting paper (using scissors)   & 31.52 & 1.35 & staple book   \\
playing with phone/tablet & 39.73 & writing   & 64.00 & 24.27 & typing on a keyboard   \\
play magic cube & 45.50 & counting money   & 65.21 & 19.71 & counting money   \\
% make victory sign & 46.48 & make ok sign   & 40.52 & -5.96 & make ok sign   \\
reading & 48.82 & writing   & 58.61 & 9.79 & writing   \\
counting money & 49.00 & play magic cube   & 50.70 & 1.70 & play magic cube   \\
blow nose & 52.04 & yawn   & 62.96 & 10.91 & yawn   \\
thumb up & 53.43 & make victory sign   & 63.30 & 9.87 & make victory sign   \\
cutting nails & 54.89 & writing   & 58.17 & 3.28 & playing with phone/tablet   \\
hit other person with something & 55.35 & wield knife towards other person   & 58.43 & 3.09 & wield knife towards other person   \\
typing on a keyboard & 56.45 & writing   & 66.18 & 9.73 & writing   \\
open a box & 56.84 & open bottle   & 65.16 & 8.32 & open bottle   \\
shoot at other person with a gun & 57.78 & point finger at the other person   & 63.83 & 6.04 & point finger at the other person   \\
fold paper & 57.96 & ball up paper   & 65.91 & 7.96 & ball up paper   \\
yawn & 58.30 & hush (quite)   & 64.00 & 5.70 & hush (quite)   \\
wield knife towards other person & 59.76 & hit other person with something   & 61.28 & 1.52 & hit other person with something   \\
pointing to something with finger & 60.96 & taking a selfie   & 72.46 & 11.51 & taking a selfie   \\
snapping fingers & 63.46 & shake fist   & 65.68 & 2.22 & shake fist   \\
open bottle & 64.10 & open a box   & 73.65 & 9.55 & play magic cube   \\
sneeze/cough & 65.30 & touch head (headache)   & 68.12 & 2.81 & touch head (headache)   \\
touch head (headache) & 65.67 & brushing teeth   & 73.91 & 8.25 & brushing teeth   \\
hush (quite) & 68.46 & yawn   & 74.17 & 5.71 & blow nose   \\
% writing & 69.96 & typing on a keyboard   & 48.90 & -21.06 & typing on a keyboard   \\
% ball up paper & 71.70 & counting money   & 70.96 & -0.74 & play magic cube   \\
touch neck (neckache) & 71.83 & touch head (headache)   & 82.25 & 10.42 & touch head (headache)   \\
flick hair & 71.87 & blow nose   & 77.74 & 5.87 & brushing hair   \\
% eat meal/snack" & 72.09 & brushing teeth   & 69.09 & -3.00 & brushing teeth   \\
drink water & 72.72 & brushing teeth   & 85.77 & 13.04 & brushing teeth   \\
shoot at the basket & 73.65 & throw   & 82.34 & 8.69 & hands up (both hands)   \\
put something into a bag & 73.78 & take something out of a bag   & 78.09 & 4.30 & take something out of a bag   \\
shake fist & 74.17 & hand waving   & 76.22 & 2.04 & hand waving   \\
throw up cap/hat & 74.57 & toss a coin   & 79.23 & 4.66 & toss a coin   \\
wipe face & 75.09 & touch head (headache)   & 87.68 & 12.59 & touch head (headache)   \\
nausea or vomiting condition & 75.36 & touch chest (stomachache/heart pain)   & 80.36 & 5.00 & touch chest (stomachache/heart pain)   \\
% sniff (smell) & 76.22 & make victory sign   & 73.39 & -2.83 & hush (quite)   \\
take off a shoe & 76.74 & wear a shoe   & 83.21 & 6.47 & wear a shoe   \\
taking a selfie & 77.26 & drink water   & 83.33 & 6.07 & pointing to something with finger   \\
knock over other person (hit with body) & 77.65 & wield knife towards other person   & 82.12 & 4.47 & wield knife towards other person   \\
% clapping & 78.12 & rub two hands together   & 78.02 & -0.10 & rub two hands together   \\
take something out of a bag & 78.17 & put something into a bag   & 82.47 & 4.30 & put something into a bag   \\
% apply cream on hand back & 78.27 & rub two hands together   & 76.66 & -1.61 & rub two hands together   \\
wear a shoe & 78.49 & take off a shoe   & 81.69 & 3.20 & take off a shoe   \\
take off headphone & 78.68 & take off glasses   & 84.98 & 6.30 & take off glasses   \\
make a phone call/answer phone & 79.00 & drink water   & 81.82 & 2.82 & playing with phone/tablet   \\
thumb down & 79.87 & thumb up   & 82.78 & 2.91 & thumb up   \\
support somebody with hand & 79.87 & follow other person   & 82.26 & 2.39 & follow other person   \\
point finger at the other person & 80.16 & pat on back of other person   & 88.41 & 8.25 & pat on back of other person   \\
reach into pocket & 80.39 & eat meal/snack"   & 83.21 & 2.82 & wear on glasses   \\
drop & 80.45 & check time (from watch)   & 83.64 & 3.18 & sniff (smell)   \\
pat on back of other person & 81.25 & point finger at the other person   & 86.96 & 5.71 & point finger at the other person   \\
tear up paper & 82.03 & fold paper   & 86.35 & 4.32 & open a box   \\
whisper in other person’s ear & 82.13 & knock over other person (hit with body)   & 86.96 & 4.83 & knock over other person (hit with body)   \\
throw & 82.27 & tennis bat swing   & 88.00 & 5.73 & wear jacket   \\
brushing teeth & 82.52 & writing   & 89.01 & 6.49 & touch head (headache)   \\
% tennis bat swing & 82.62 & throw up cap/hat   & 78.75 & -3.88 & throw up cap/hat   \\
put on headphone & 82.96 & wear on glasses   & 87.52 & 4.57 & wear on glasses   \\
check time (from watch) & 83.42 & eat meal/snack"   & 89.49 & 6.07 & rub two hands together   \\
step on foot & 83.52 & kicking other person   & 86.26 & 2.74 & kicking other person   \\
\bottomrule 
\end{tabular}
}
\label{table:velocity_complete_action_imp_1}
\end{table*}

\begin{table*}[t]
% Second Half 
\caption{Velocity: Second Half. }
\resizebox{\textwidth}{!}{
\begin{tabular}{l|rc|rrc}
\toprule 
%\rowcolor{Gray}
 & \multicolumn{2}{c|}{\textbf{Joint}} & \multicolumn{3}{c}{\textbf{Concatenation: Joint + Angular}} \\
\cline{2-3}\cline{4-6}
%\rowcolor{Gray}
\multirow{-2}{*}{\textbf{Action}} & Acc (\%) & Similar Action & Acc (\%) & Acc$\uparrow$ (\%) & Similar Action \\ 
\midrule 
% \rowcolor{Gray!30}
grab other person’s stuff & 83.52 & wield knife towards other person   & 87.30 & 3.78 & touch other person's pocket   \\
toss a coin & 83.99 & thumb up   & 86.56 & 2.57 & snapping fingers   \\
brushing hair & 84.35 & brushing teeth   & 87.91 & 3.56 & use a fan (with hand or paper)/feeling warm   \\
shake head & 84.45 & typing on a keyboard   & 92.73 & 8.27 & touch neck (neckache)   \\
cross hands in front (say stop) & 84.51 & put the palms together   & 90.58 & 6.07 & put the palms together   \\
take a photo of other person & 84.59 & shoot at other person with a gun   & 90.10 & 5.51 & shoot at other person with a gun   \\
% apply cream on face & 85.06 & eat meal/snack"   & 81.71 & -3.36 & wipe face   \\
move heavy objects & 86.15 & carry something with other person   & 89.96 & 3.82 & carry something with other person   \\
take off bag & 86.15 & take off jacket   & 90.97 & 4.82 & take off jacket   \\
cheer up & 86.23 & hand waving   & 89.42 & 3.19 & use a fan (with hand or paper)/feeling warm   \\
use a fan (with hand or paper)/feeling warm & 86.27 & hand waving   & 88.36 & 2.09 & shake fist   \\
% rub two hands together & 86.32 & clapping   & 85.87 & -0.45 & clapping   \\
put on a hat/cap & 86.50 & wear on glasses   & 96.32 & 9.82 & wear on glasses   \\
punching/slapping other person & 86.59 & hit other person with something   & 86.86 & 0.27 & hit other person with something   \\
nod head/bow & 86.68 & touch chest (stomachache/heart pain)   & 94.93 & 8.25 & take off a shoe   \\
hand waving & 86.96 & use a fan (with hand or paper)/feeling warm   & 90.15 & 3.19 & use a fan (with hand or paper)/feeling warm   \\
% giving something to other person & 87.04 & exchange things with other person   & 86.23 & -0.81 & exchange things with other person   \\
touch back (backache) & 87.41 & touch chest (stomachache/heart pain)   & 91.30 & 3.90 & touch chest (stomachache/heart pain)   \\
put on bag & 87.52 & take off jacket   & 93.22 & 5.70 & wear jacket   \\
exchange things with other person & 87.52 & giving something to other person   & 88.52 & 1.00 & giving something to other person   \\
salute & 87.77 & kicking something   & 90.22 & 2.45 & brushing teeth   \\
cross toe touch & 87.85 & move heavy objects   & 89.37 & 1.52 & move heavy objects   \\
wear on glasses & 88.01 & eat meal/snack"   & 92.67 & 4.66 & brushing hair   \\
hands up (both hands) & 88.72 & stretch oneself   & 91.29 & 2.57 & stretch oneself   \\
touch chest (stomachache/heart pain) & 89.22 & touch back (backache)   & 90.22 & 1.00 & touch back (backache)   \\
touch other person's pocket & 89.55 & pat on back of other person   & 93.82 & 4.27 & giving something to other person   \\
put the palms together & 89.58 & check time (from watch)   & 90.94 & 1.36 & cross hands in front (say stop)   \\
cross arms & 90.13 & cross hands in front (say stop)   & 94.43 & 4.30 & put the palms together   \\
kicking other person & 90.30 & kicking something   & 91.30 & 1.00 & punching/slapping other person   \\
take off glasses & 90.97 & wear on glasses   & 92.70 & 1.73 & take off headphone   \\
pickup & 91.00 & take off a shoe   & 93.82 & 2.82 & take off a shoe   \\
hopping (one foot jumping) & 91.36 & running on the spot   & 96.73 & 5.36 & staggering   \\
juggling table tennis balls & 91.50 & open a box   & 94.42 & 2.92 & open a box   \\
pushing other person & 91.75 & punching/slapping other person   & 93.84 & 2.09 & touch other person's pocket   \\
bounce ball & 91.98 & juggling table tennis balls   & 93.51 & 1.53 & finger-guessing game (playing rock-paper-scissors)   \\
% stretch oneself & 92.23 & taking a selfie   & 91.15 & -1.08 & hands up (both hands)   \\
side kick & 92.55 & kicking something   & 94.95 & 2.39 & kicking something   \\
high-five & 92.58 & finger-guessing game (playing rock-paper-scissors)   & 95.66 & 3.08 & make victory sign   \\
carry something with other person & 92.75 & support somebody with hand   & 94.44 & 1.69 & support somebody with hand   \\
sitting down & 92.77 & falling   & 93.04 & 0.27 & nod head/bow   \\
butt kicks (kick backward) & 93.08 & side kick   & 95.30 & 2.22 & side kick   \\
% finger-guessing game (playing rock-paper-scissors) & 93.10 & use a fan (with hand or paper)/feeling warm   & 92.36 & -0.74 & use a fan (with hand or paper)/feeling warm   \\
handshaking & 93.20 & hugging other person   & 95.65 & 2.45 & pat on back of other person   \\
wear jacket & 93.55 & take off jacket   & 97.09 & 3.55 & take off jacket   \\
take off a hat/cap & 93.87 & take off glasses   & 95.24 & 1.37 & shake head   \\
% walking apart from each other & 94.29 & walking towards each other   & 93.84 & -0.45 & walking towards each other   \\
% follow other person & 94.49 & walking apart from each other   & 93.92 & -0.56 & walking apart from each other   \\
falling & 94.64 & squat down   & 97.09 & 2.45 & staggering   \\
squat down & 94.82 & sitting down   & 96.86 & 2.05 & sitting down   \\
jump up & 95.38 & running on the spot   & 98.19 & 2.81 & hopping (one foot jumping)   \\
% kicking something & 96.10 & standing up (from sitting position)   & 94.93 & -1.17 & side kick   \\
cheers and drink & 96.22 & grab other person’s stuff   & 97.39 & 1.17 & high-five   \\
% walking towards each other & 96.44 & walking apart from each other   & 94.14 & -2.30 & walking apart from each other   \\
staggering & 96.46 & kicking something   & 97.83 & 1.36 & walking towards each other   \\
running on the spot & 96.74 & bounce ball   & 97.04 & 0.30 & hopping (one foot jumping)   \\
hugging other person & 96.81 & check time (from watch)   & 98.18 & 1.36 & check time (from watch)   \\
arm swings & 96.91 & arm circles   & 97.91 & 1.00 & arm circles   \\
arm circles & 97.43 & stretch oneself   & 98.78 & 1.35 & stretch oneself   \\
% take off jacket & 97.55 & wear jacket   & 97.10 & -0.45 & wear jacket   \\
% standing up (from sitting position) & 97.90 & wear a shoe   & 96.34 & -1.56 & wear a shoe   \\
\bottomrule 
\end{tabular}
}
\label{table:velocity_complete_action_imp_2}
\end{table*}


==> secs/tables/old_diff_ang_imp_table.tex <==
\begin{table*}[htbp]
\caption{
A comparison of the effect for improving action recognition by concatenating certain angular feature to the joint representation. Each subtable is sorted by the increase of accuracy.  
The `Action' column shows the ground truth labels, and the `Similar Action' column shows the predictions from the model (with/without angular features).
The accuracy improvements highlighted in red are the substantially increased ones (Acc$\uparrow$ $\geq$ 10\%) due to using our angular features.
} 
% \vspace{-2mm}
% Subtable 1
% \caption{Actions whose accuracy values are boosted by the local angular feature. }
% \resizebox{\textwidth}{!}{
\begin{tabular}{c|l|rc|rrc}
\toprule 
%\rowcolor{Gray}
& & \multicolumn{2}{c|}{\textbf{Joint}} & \multicolumn{3}{c}{\textbf{Concatenation: Joint + Angular}} \\
\cline{3-4}\cline{5-7}
%\rowcolor{Gray}
& \multirow{-2}{*}{\textbf{Action}} & Acc (\%) & Similar Action & Acc (\%) & Acc$\uparrow$ (\%) & Similar Action \\ 
\midrule 
\multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{Static}}} 
& take off a shoe & 72.63 & wear a shoe & 80.67 & 12.04 & wear a shoe \\
& use a fan &	83.27 & hand waving & 90.55	& 7.27 & shake fist \\
& staple book & 27.32 & cutting paper & 36.08 & 8.76 & cutting paper \\
& fold paper & 60.35 & ball up paper & 66.78 & 6.43 & open a box \\
& counting money & 47.72 & play magic cube & 54.04 & 6.32 & play magic cube \\
& take off headphone & 80.04 & take off glasses & 85.87 & 5.83 & take off glasses \\
& kicking other person & 86.04 & step on foot & 91.3 & 5.26 & side kick \\
% & wield knife towards other person & 64.24 & hit other person with something & 68.92 & 4.69 & hit other person with something \\
% & pointing to something with finger & 72.46 & taking a selfie & 76.45 & 3.99 & taking a selfie \\
% & touch head & 78.26 & brushing teeth & 81.88 & 3.62 & blow nose \\
\midrule
\multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{Velocity}}} 
% & make victory sign & 36.87 & make ok sign & 49.22 & 12.35 & make ok sign \\
& cutting paper (using scissors) & 35.78 & staple book & 45.90 & 10.12 & staple book \\
& writing & 54.04 & typing on a keyboard & 61.76 & 7.72 & typing on a keyboard \\
& drop & 78.18 & sniff (smell) & 84.73 & 6.55 & sniff (smell) \\
& fold paper & 57.22 & ball up paper & 63.48 & 6.26 & counting money \\
& take a photo of other person & 84.03 & shoot at other person with a gun & 89.93 & 5.9 & shoot at other person with a gun \\
& typing on a keyboard & 61.82 & writing & 67.27 & 5.45 & writing \\
& wear on glasses & 86.78 & eat meal/snack & 91.94 & 5.16 & eat meal/snack \\
\bottomrule % Table 2
\toprule 
& & \multicolumn{2}{c|}{\textbf{Joint}} & \multicolumn{3}{c}{\textbf{Concatenation: Joint + Angular}} \\
\cline{3-4}\cline{5-7}
%\rowcolor{Gray}
& \multirow{-2}{*}{\textbf{Action}} & Acc (\%) & Similar Action & Acc (\%) & Acc$\uparrow$ (\%) & Similar Action \\ 
\midrule 
\multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{Static}}} 
& make victory sign & 17.22 & make ok sign & 40.35 & 23.13 & make ok sign \\ 
& playing with phone/tablet & 54.55 & play magic cube & 68.36 & 13.82 & play magic cube \\
& take something out of a bag & 78.3 & put something into a bag & 85.94 & 7.64 & put something into a bag \\
& fold paper & 59.83 & open a box & 66.09 & 6.26 & counting money \\
& counting money & 45.26 & play magic cube & 51.4 & 6.14 & play magic cube \\
& open bottle & 65.97 & play magic cube & 71.9 & 5.93 & play magic cube \\
& brushing hair & 86.45 & touch head & 91.94 & 5.49 & wipe face \\
% & brushing teeth & 79.49 & touch head & 84.62 & 5.13 & drink water \\
% & typing on a keyboard & 61.45 & writing & 66.55 & 5.09 & writing \\
% & exchange things with other person & 85.74 & giving something to other person & 89.91 & 4.17 & giving something to other person \\ \bottomrule 
\midrule 
\multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{Velocity}}} 
& cutting paper (using scissors) & 35.78 & staple book & 58.12 & 22.34 & staple book \\
& check time (from watch) & 80.43 & cross hands in front (say stop) & 89.49 & 9.06  & tear up paper \\
& typing on a keyboard & 61.82 & writing & 70.18 & 8.36 & writing \\
& open bottle & 65.1 & open a box & 72.43 & 7.33 & open a box \\
& counting money & 46.84 & play magic cube & 53.86 & 7.02 & play magic cube \\
& open a box & 59.23 & open bottle & 65.16 & 5.92 & open bottle \\
& drink water & 82.12 & make a phone call & 87.96 & 5.84 & brushing teeth \\
\bottomrule
\toprule % Table 3
%\rowcolor{Gray}
& & \multicolumn{2}{c|}{\textbf{Joint}} & \multicolumn{3}{c}{\textbf{Concatenation: Joint + Angular}} \\
\cline{3-4}\cline{5-7}
%\rowcolor{Gray}
& \multirow{-2}{*}{\textbf{Action}} & Acc (\%) & Similar Action & Acc (\%) & Acc$\uparrow$ (\%) & Similar Action \\ 
\midrule
\multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{Static}}} 
& make victory sign & 17.22 & make ok sign & 37.39 & 20.17 & make ok sign \\
% nausea or vomiting condition & 76.36 & touch chest (stomachache/heart pain) & 86.18 & 9.82 & touch chest (stomachache/heart pain) \\
& counting money & 45.26 & play magic cube & 54.56 & 9.3 & play magic cube \\
& brushing teeth & 79.49 & touch head (headache) & 88.28 & 8.79 & drink water \\
& shake fist & 71.7 & hand waving & 78.47 & 6.77 & hand waving \\ 
& hopping (one foot jumping) & 92 & staggering & 96.73 & 4.73 & staggering \\
& hit other person with something & 58.61 & wield knife towards other person & 63.13 & 4.52 & wield knife towards other person \\
& grab other person's stuff & 85.39 & wield knife towards other person & 89.91 & 4.52 & hit other person with something \\
% & take something out of a bag & 78.3 & put something into a bag & 81.94 & 3.65 & put something into a bag \\
% & pointing to something with finger & 73.55 & taking a selfie & 77.17	& 3.62 & taking a selfie \\
% & take off jacket & 92.39 & take off bag & 96.01 & 3.62 & wear jacket \\
\midrule
\multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{Velocity}}}
& cutting paper (using scissors) & 35.78 & staple book & 59.34 & 23.56 & staple book  \\
& brushing teeth & 77.29 & drink water & 88.28 & 10.99 & drink water \\
& check time (from watch) & 80.43 & cross hands in front (say stop) & 90.94 & 10.51 & taking a selfie \\
& typing on a keyboard & 61.82 & writing & 72.00 & 10.18 & writing \\
& open a box & 59.23 & open bottle & 68.82 & 9.58 & open bottle \\
& play magic cube & 58.57 & playing with phone/tablet & 64.86 & 6.29 & counting money \\
& hand waving & 87.16 & shake fist & 93.43 & 6.27 & use a fan \\
\bottomrule 
\toprule % Table 4
%\rowcolor{Gray}
& & \multicolumn{2}{c|}{\textbf{Joint}} & \multicolumn{3}{c}{\textbf{Concatenation: Joint + Angular}} \\
\cline{3-4}\cline{5-7}
%\rowcolor{Gray}
& \multirow{-2}{*}{\textbf{Action}} & Acc (\%) & Similar Action & Acc (\%) & Acc$\uparrow$ (\%) & Similar Action \\ 
\midrule
\multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{Static}}} 
& make victory sign & 17.22 & make ok sign & 47.13 & 29.91 & thumb up \\
& shake fist & 71.70 & hand waving & 80.56 & 8.85 & hand waving \\ 
& counting money & 45.26 & play magic cube & 52.63 & 7.37 & play magic cube \\
& snapping fingers & 58.54 & thumb up & 65.68 & 7.14 & shake fist \\
& pointing to something with finger & 73.55 & taking a selfie & 80.43 & 6.88 & taking a selfie \\
& exchange things with other person & 85.74 & giving something to other person & 89.91 & 6.87 & giving something to other person \\
& open bottle & 65.97 & play magic cube & 72.6 & 6.63 & play magic cube \\
% eat meal & 67.27 & drink water & 73.09 & 5.82 & brushing teeth \\
% brushing teeth & 79.49 & touch head (headache) & 84.98 & 5.49 & 	touch head (headache) \\ 
% playing with phone/tablet & 54.55 & play magic cube & 60 & 5.45 & 	apply cream on hand back \\
% cutting paper (using scissors) & 62.13 & staple book & 66.84 & 4.71 & staple book \\
% hit other person with something & 58.61 & wield knife towards other person & 62.96 & 4.35 & wield knife towards other person \\
\midrule
\multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{Velocity}}}
& cutting paper (using scissors) & 35.78 & staple book & 53.4 & 17.63 & staple book \\
& typing on a keyboard & 61.82 & writing & 74.18 & 12.36 & writing \\
& ball up paper & 68 & counting money & 77.91 & 9.91 & counting money \\
& brushing teeth & 77.29 & drink water & 86.81 & 9.52 & touch head (headache) \\
& snapping fingers & 59.58 & thumb up & 68.47 & 8.88 & thumb up \\
& pointing to something with finger & 70.29 & take a selfie & 78.26 & 7.97 & take a selfie \\
& play magic cube & 58.57 & playing with phone &	64.86 & 6.29 & counting money \\
\bottomrule 
\end{tabular}
% }
\label{table:diff_angle_analysis}
\end{table*}

